Near Optimal Parallel Algorithms for Dynamic DFS in Undirected Graphs

Depth first search (DFS) tree is a fundamental data structure for solving graph problems. The classical algorithm [SiComp74] for building a DFS tree requires $O(m+n)$ time for a given graph $G$ having $n$ vertices and $m$ edges. Recently, Baswana et al. [SODA16] presented a simple algorithm for updating DFS tree of an undirected graph after an edge/vertex update in $\tilde{O}(n)$ time. However, their algorithm is strictly sequential. We present an algorithm achieving similar bounds, that can be adopted easily to the parallel environment. In the parallel model, a DFS tree can be computed from scratch using $m$ processors in expected $\tilde{O}(1)$ time [SiComp90] on an EREW PRAM, whereas the best deterministic algorithm takes $\tilde{O}(\sqrt{n})$ time [SiComp90,JAlg93] on a CRCW PRAM. Our algorithm can be used to develop optimal (upto polylog n factors deterministic algorithms for maintaining fully dynamic DFS and fault tolerant DFS, of an undirected graph. 1- Parallel Fully Dynamic DFS: Given an arbitrary online sequence of vertex/edge updates, we can maintain a DFS tree of an undirected graph in $\tilde{O}(1)$ time per update using $m$ processors on an EREW PRAM. 2- Parallel Fault tolerant DFS: An undirected graph can be preprocessed to build a data structure of size O(m) such that for a set of $k$ updates (where $k$ is constant) in the graph, the updated DFS tree can be computed in $\tilde{O}(1)$ time using $n$ processors on an EREW PRAM. Moreover, our fully dynamic DFS algorithm provides, in a seamless manner, nearly optimal (upto polylog n factors) algorithms for maintaining a DFS tree in semi-streaming model and a restricted distributed model. These are the first parallel, semi-streaming and distributed algorithms for maintaining a DFS tree in the dynamic setting.

==> heavySp.tex <==
%\section{Special case of heavy subtree traversal}
\subsubsection*{Special case of heavy subtree traversal}
\label{sec:SpecialCase}
In this section $(x_p,y_p)$ and $(x_r,y_r)$ correspond to the back edges used in 
$p$ and $r$ traversals described earlier,
%in Section~\ref{sec:heavyP}, 
whereas $(x_{p'},y_{p'})$ and $(x_{r'},y_{r'})$ correspond the back edges used in modified $p'$
and $r'$ traversals described below. 
%In this entire section $(x_p,y_p)$ and $(x_r,y_r)$ correspond to the  back edges used in 
%$p$ and $r$ traversals described in Section~\ref{sec:heavyP}, where as 
%$(x_{p'},y_{p'})$ and $(x_{r'},y_{r'})$ would correspond the  back edges used in modified $p'$
%and $r'$ traversals described below. 
Our modified $p'$ traversal and $r'$ traversal would use 
$(x_{p'},y_{p'})=(x_3,y_3)$ and $(x_{r'},y_{r'})=(x_2,y_2)$ respectively, 
which will be followed by an appropriate traversal (see Figure \ref{fig:pdfsSp}).
We now recall the conditions leading to the {\em special} case, 
and describe its implications on $(x_p,y_p)$, $(x_r,y_r)$ and $(x_d,y_d)$
(see Appendix~\ref{sec:proofs} for proof).
%We now recall the conditions leading to the {\em special} case its implications on
%$(x_p,y_p)$, $(x_r,y_r)$ and $(x_d,y_d)$.

\begin{lemma}
	The conditions of the special case are (i) $x_3\in T(v_R)$, (ii) $x_p\in \tau_d$, and 
	(iii) $(x_r,y_r)=(x'_2,y'_2)$. Following are the properties of $(x_p,y_p)$ and $(x_d,y_d)$ 
	in this case.
	\begin{enumerate}
\item $y_d=y_p$,$y_3$ is lower than $y_d$ on $path(r_c,r')$, and $y_r$ is lower than $y_2$ on $path(r_c,r')$.
\item No subtree of $\tau_d$ hanging from $path(root(\tau_d),x_p)$, with an edge to $p_c$, 
		has an edge lower than $y_2$ on $path(r_c,r')$. %\label{obs:disconTd}
\item No subtree of $\tau_d$ hanging from $path(root(\tau_d),x_r)$, with an edge to $p_c$,
		has an edge higher than $y_3$ on $path(r_c,r')$. 	%\label{obs:disconTdx}
	\end{enumerate}			
	\label{lem:propSC}
\end{lemma}
%\begin{proof}
%Recall the choice of $(x_d,y_d)$ and $(x_p,y_p)$ (see Appendix~\ref{sec:choose_ep_ed}), it was the highest edge from 
%$\tau_d$ on $path(r_c,r')$ and $(x_p,y_p)$ was computed such that $y_p\in path(y_d,r')$. 
%Hence, if $x_p\in \tau_d$ we necessarily have $y_d=y_p$.
%Also, $y_3$ is strictly lower than $y_p$ (or $y_d$) else having a lower $LCA(x_3,v_H)$ 
%than $LCA(x_p,v_H)$, $(x_3,y_3)$ would have been selected as $(x_p,y_p)$ earlier.
%Finally, $y_2$ is strictly higher than $y_r$ otherwise $(x_2,y_2)$ 
%would have been selected as $(x_r,y_r)$ earlier.
%Second property holds since $(x_2,y_2)$ (where $x_2\in T(v_P)$) was the lowest edge on $path(r_c,r')$
%from the eligible subtrees after $p$ traversal. 
%Third property holds since $(x_3,y_3)$ (where $x_3\in T(v_R)$) was the highest edge on $path(r_c,r')$
%from the eligible subtrees after $r$ traversal.
%\end{proof}


\begin{figure*}[!ht]
	\centering
	\includegraphics[width=.9\linewidth]{Figures/pdfs_egSp.pdf}
	\caption{The three scenarios for {\em special case} of Heavy Subtree Traversal
		shown (using blue dotted lines) 
		(a) Modified $p'$ traversal with $(x_{p'},y_{p'})=(x_3,y_3)$,
		(b) Modified $r'$ traversal with $(x_{r'},y_{r'})=(x_2,y_2)$, 
		(c) Residual $r'$ traversal with $(x_{r'},y_{r'})=(x_2,y_2)$.		
	}
	\label{fig:pdfsSp}
\end{figure*}

To handle this special case, we again check the scenario's corresponding to $p$ and $r$ traversals 
ignoring the {\em eligible} subtree $\tau_d$. Hence, the corresponding edges $(x_{p'},y_{p'})$ and $(x_{r'},y_{r'})$
for these scenarios does not emerge from $\tau_d$.  Thus, ignoring $\tau_d$, for each traversal 
the first two conditions of {\em applicability} lemma would be satisfied. In case this traversal can be 
followed by the traversal of $\tau_d$ such that {\em applicability} lemma is satisfied, 
it is performed else we move to the next traversal.

\subsection*{Modified {\large $p'$} traversal}
Consider a modified $p'$ traversal using $(x_{p'},y_{p'})=(x_3,y_3)$ %instead of a higher $(x_p,y_p)$ 
as shown in Figure~\ref{fig:pdfsSp} (a), traversing the path 
$p^*_{P'}=path(r_c,x_3)\cup (x_3,y_3)\cup path(y_3,par(v_l))$ 
%T(see Figure~\ref{fig:pdfsSp} (a)). 
This leaves an un-traversed part of $path(r_c,r')$, say $p_1=path(par(y_3),r')$, 
that necessarily contains $y_d$ as $y_3$ is strictly lower than $y_d$ (see Lemma~\ref{lem:propSC}).
%This is because $y_3$ is strictly lower than $y_p$ (or $y_d$) else having a lower $LCA(x_3,v_H)$ 
%than $LCA(x_p,v_H)$, $(x_3,y_3)$ would have been selected as $(x_p,y_p)$ earlier.
Now, the computation of $(x_3,y_3)$ ensures that no {\em eligible} subtree (except for $\tau_d$)
is connected to both paths $p_1$ and $p_c$, as well as ensuring that $T(v_{P'})$ is not connected to $p_1$. 
This satisfies the first two conditions of {\em applicability} lemma ignoring $\tau_d$.
Since, $\tau_d$ is necessarily connected to two paths $p_1$ and $p_c$, its component will not be of 
type $C1$ or $C2$, which is not permissible.

%Thus, the subtree $\tau_d$ is connected to two paths $p_1$ and $p_c$, which is also the only subtree
%connected to both $p_1$ and $p_c$ (recall computation of $(x_3,y_3)$). 
%This is not permissible as the component having $\tau_d$ will not be of 
%type $C1$ or $C2$. 
%
%This is clearly not permissible as the component having $\tau_d$ and $p_c$ will not be of 
%type $C1$ or $C2$. 

However, if this traversal is followed by the traversal of $p_{P'}=(y_r,x_r)\cup (x_r,root(\tau_d))$
(see Figure~\ref{fig:pdfsSp} (a)), no subtree of $\tau_d$ hanging from $p_{P'}$ is connected to both
$p_c$ and $p_1$ (see property~3 in Lemma~\ref{lem:propSC}). 
This satisfies the first two conditions of {\em applicability} lemma.
Also, since $T(v_{P'})$ does not have an edge to $\tau_d$, after this traversal the component 
having $p_c$ would have the new root in $\tau_d$ or $p_c$, satisfying the third condition 
of {\em applicability} lemma. 
Thus, if the lowest edge on $p^*_{P'}$ from the component containing $p_c$ is from $\tau_d$,
i.e. $(x_r,y_r)$, the traversal of $p^*_{P'}$ followed by $p_{P'}$, 
satisfies {\em applicability} lemma. Clearly no subtree hanging from $p^*_{P'}$ has an
edge to both $p_c$ and $p_1$ as $y_2$ is higher than $y_r$ on $path(r_c,r')$ (Lemma~\ref{lem:propSC}).
Note that even though the only subtree with an edge to both $p_c$ and $p_1$ is $\tau_d$,
the path $p_1$ and subtrees connected to it are also in the component containing $p_c$.
Thus, the lowest edge on $p^*_{P'}$ may not always be from $\tau_d$.

\begin{remark}
%Since the lowest edge from the {\em eligible} subtrees on $path(r_c,r')$ is $(x_r,y_r)=(x'_2,y'_2)$,
	This traversal is not applicable only if there is an edge lower than $y_r$ on $path(r_c,r')$, 
	from $p_1$ or some subtree connected to $p_1$.
	% (not directly to $p_c$).
\end{remark}

\subsection*{Modified {\large $r'$} traversal}
Consider a modified $r'$ traversal using $(x_{r'},y_{r'})=(x_2,y_2)$ %instead of a lower $(x_r,y_r)$
traversing the path $p^*_{R'}=path(r_c,x_{r'})\cup (x_{r'},y_{r'})\cup path(y_{r'},r')$ 
(see Figure~\ref{fig:pdfsSp} (b)). 
This leaves an un-traversed part of $path(r_c,r')$, say $p_2=path(par(v_l),y_2)\backslash\{y_2\}$,
that necessarily contains $y_r$ 
as $y_2$ is strictly higher than $y_r$ (see Lemma~\ref{lem:propSC}).
%. This is because $y_2$ is strictly higher than $y_r$
%otherwise $(x_2,y_2)$ would have been selected as $(x_r,y_r)$ earlier.
Now, the computation of $(x_2,y_2)$ ensures that no {\em eligible} subtree (except for $\tau_d$)
is connected to both paths $p_2$ and $p_c$, as well as ensuring that $T(v_{R'})$ is not connected to $p_2$. 
This satisfies the first two conditions of {\em applicability} lemma ignoring $\tau_d$.
Since, $\tau_d$ is necessarily connected to two paths $p_2$ and $p_c$, its component will not be of 
type $C1$ or $C2$, which is not permissible.
%Thus, the subtree $\tau_d$ is connected to two paths $p_2$ and $p_c$, which is also the only subtree
%connected to both $p_2$ and $p_c$ (recall computation of $(x_2,y_2)$). 
%This is not permissible as the component having $\tau_d$ will not be of 
%type $C1$ or $C2$. 
%%This is clearly not permissible as the component having $\tau_d$ and $p_c$ will not be of 
%%type $C1$ or $C2$. 

However, if this traversal is followed by the traversal of $p_{R'}=(y_p,x_p)\cup (x_p,root(\tau_d))$
(see Figure~\ref{fig:pdfsSp} (b)), 
no subtree of $\tau_d$ hanging from $p_{R'}$ is connected to both
$p_c$ and $p_2$ (see property~2 in Lemma~\ref{lem:propSC}).
This satisfies the first two conditions of {\em applicability} lemma.
Also, since $T(v_{R'})$ does not have an edge to $\tau_d$, after this traversal the component 
having $p_c$ would have the new root in $\tau_d$ or $p_c$, satisfying the third condition 
of {\em applicability} lemma. 
%Also, since $\tau_d$ is connected to $p_c$, after this traversal the component 
%having $p_c$ would have the new root in $\tau_d$, satisfying the third condition 
%of {\em applicability} lemma. 
Thus, if the lowest edge on $p^*_{R'}$ from the component containing $p_c$ 
is from $\tau_d$, i.e. $(x_p,y_p)$, the traversal of $p^*_{R'}$ followed by $p_{R'}$, 
satisfies {\em applicability} lemma. Clearly no subtree hanging from $p^*_{R'}$ has an
edge to both $p_c$ and $p_2$ as $y_3$ is lower than $y_d$ on $path(r_c,r')$ (Lemma~\ref{lem:propSC}).
Note that even though the only subtree with an edge to both $p_c$ and $p_2$ is $\tau_d$,
the path $p_2$ and subtrees connected to it are also in the component containing $p_c$.
Thus, the lowest edge on $p^*_{R'}$ may not always be from $\tau_d$.

\begin{remark}
%	Since the highest edge from the {\em eligible} subtrees on $path(r_c,r')$ is $(x_p,y_p)$,
	This traversal is not applicable only if there is an edge higher than $y_p$ on $path(r_c,r')$, 
	from $p_2$ or some subtree connected to $p_2$. % and not $p_c$.
\end{remark}

\subsection*{Residual {\large $r''$} traversal}
The remarks of modified $p'$ traversal and modified $r'$ traversal show that 
$path(par(v_l),y_r)\backslash\{y_r\}$ (say $p_3$) and $path(par(y_p),r')$ (say $p_4$)
are connected either directly by an edge or some subtree $\tau'$ having edge to both $p_3$ and $p_4$ 
and not to $p_c$ (see Figure~\ref{fig:pdfsSp} (c)). Let the lowest such edge on $p_3$ be 
$(x',y')$ (if directly connected) or $(y_{\tau'},y')$ (if connected via $\tau'$) 
where $y'\in p_3$. In the latter case let the highest edge from $\tau'$ on $p_4$ 
be $(x',x_{\tau'})$.  
In both cases, we call this path from $x'$ to $y'$ as $p_{\tau'}$, i.e.,
$p_{\tau'}=(x',y')$ or $p_{\tau'}=(x',x_{\tau'})\cup path(x_{\tau'},y_{\tau'})\cup (y_{\tau'},y')$.

We perform the traversal shown in Figure~\ref{fig:pdfsSp} (c), where 
$p^*_{R''}=path(r_c,x_2)\cup (x_2,y_2)\cup path(y_2,x')\cup p_{\tau'}\cup path(y',y_2)\backslash\{y_2\}$.
As a result, we may have four unvisited paths, 
(i) in unvisited part of $\tau'$, 
(ii) $path(par(x'),r')$ (say $p'_4$), 
(iii) $path(par(v_l),y')\backslash\{y'\}$ (say $p'_3$), 
and (iv) $p_c$.
Now, (i) the unvisited part of $\tau'$ is not connected to $p_c$ (see remark in $p'$ and $r'$ traversal) and 
$p'_3$ or $p'_4$ (by construction) which forms a separate component. 
Also, (ii) any subtree connected to $p'_4$ is not connected to $p'_3$ 
($y'$ corresponds to the lowest such edge on $p_3$) which is also not connected to $\tau_d$ and hence $p_c$ 
(as $y_d\notin p'_4$). 
Further, (iii) $p'_3$ is also not connected to $\tau_d$ and hence $p_c$ (as $y_r\notin p'_3$). 
%Also, any subtree connected to $p'_4$ is not connected to $p'_3$ ($y'$ corresponds to the lowest such edge on $p_3$). 
%Further, subtree $\tau_d$ (and hence any subtree connected to $p_c$) is not connected to $p'_3$ or $p'_4$ 
%(as $y_r\notin p'_3$ and $y_p\notin p'_4$).
Finally, (iv) the component having $p_c$ will have the new root in $\tau_d$, 
which is not a heavy subtree. Hence, the traversal of $p^*_{R''}$ 
satisfies {\em applicability} lemma. Refer to Procedure~\ref{alg:dfs_c2sp} in 
Appendix~\ref{appn:pseudocode} for  pseudo code.


==> heavySp2.tex <==
\section{Special case of heavy subtree traversal}
\label{sec:SpecialCase}
In this entire section $(x_p,y_p)$ and $(x_r,y_r)$ correspond to the  back edges used in 
$p$ and $r$ traversals described in Section~\ref{sec:heavyP}, whereas $(x_{r'},y_{r'})$ would 
correspond the back edge used in the modified $r'$ traversal described as follows.
To handle this special case, we again check the scenario corresponding to $r$ traversal 
ignoring the {\em eligible} subtree $\tau_d$. Hence, the corresponding back edge 
$(x_{r'},y_{r'})$ does not emerge from $\tau_d=\tau_p$, i.e., $(x_{r'},y_{r'})=(x_2,y_2)$.  
Thus, ignoring $\tau_d$, the first two conditions of Lemma~\ref{lem:non-applicable} would be satisfied. 
We show that this traversal can be followed by either by a disconnecting traversal of $\tau_d$ 
or some non-eligible subtree $\tau'$ such that Lemma~\ref{lem:non-applicable} is satisfied. 

\begin{figure*}[!ht]
	\centering
	\includegraphics[width=.6\linewidth]{Figures/pdfs_egSp2.pdf}
	\caption{The two types of {\em special case} of Heavy Subtree Traversal
		shown (using blue dotted lines) 
		(a) Modified $r'$ traversal with disconnecting traversal of $\tau_d$, 
		(b) Modified $r'$ traversal with disconnecting traversal of $\tau'$. 
	}
	\label{fig:pdfsSp}
\end{figure*}



\subsection*{Modified {\large $r'$} traversal}
Consider a modified $r'$ traversal using $(x_{r'},y_{r'})=(x_2,y_2)$ instead of a 
lower $(x_r,y_r)$ traversing the path 
$p^*_{R'}=path(r_c,x_{r'})\cup (x_{r'},y_{r'})\cup path(y_{r'},r')$ 
(see Figure~\ref{fig:pdfsSp} (b)). 
This leaves an un-traversed part of $path(r_c,r')$, say $p_2=path(par(v_l),y_2)\backslash\{y_2\}$,
that necessarily contains $y_r$ as $y_2$ is strictly higher than $y_r$ (see Lemma~\ref{lem:propSC}).
%. This is because $y_2$ is strictly higher than $y_r$
%otherwise $(x_2,y_2)$ would have been selected as $(x_r,y_r)$ earlier.
Now, the computation of $(x_2,y_2)$ ensures that no {\em eligible} subtree (except for $\tau_d$)
is connected to both paths $p_2$ and $p_c$, as well as ensuring that $T(v_{R'})$ is not connected to $p_2$. 
This satisfies the first two conditions of Lemma~\ref{lem:non-applicable} ignoring $\tau_d$.
Since, $\tau_d$ is necessarily connected to two paths $p_2$ and $p_c$, its component will not be of 
type $C1$ or $C2$, which is not permissible.
%Thus, the subtree $\tau_d$ is connected to two paths $p_2$ and $p_c$, which is also the only subtree
%connected to both $p_2$ and $p_c$ (recall computation of $(x_2,y_2)$). 
%This is not permissible as the component having $\tau_d$ will not be of 
%type $C1$ or $C2$. 
%%This is clearly not permissible as the component having $\tau_d$ and $p_c$ will not be of 
%%type $C1$ or $C2$. 

However, if this traversal is followed by the traversal of $p_{R'}=(y_p,x_p)\cup (x_p,root(\tau_d))$
(see Figure~\ref{fig:pdfsSp} (b)), no subtree of $\tau_d$ connected to $p_c$ will be connected to 
$p_2$ (see property~2 in Lemma~\ref{lem:propSC}). 
This satisfies the first two conditions of Lemma~\ref{lem:non-applicable}.
Also, since $T(v_{R'})$ does not have an edge to $\tau_d$, after this traversal the component 
having $p_c$ would have the new root in $\tau_d$ or $p_c$, satisfying the third condition 
of Lemma~\ref{lem:non-applicable}. 
%Also, since $\tau_d$ is connected to $p_c$, after this traversal the component 
%having $p_c$ would have the new root in $\tau_d$, satisfying the third condition 
%of Lemma~\ref{lem:non-applicable}. 
Thus, if the lowest edge on $p^*_{R'}$ from the component containing $p_c$ 
is from $\tau_d$, i.e. $(x_p,y_p)$, the traversal of $p^*_{R'}$ followed by $p_{R'}$, 
satisfies Lemma~\ref{lem:non-applicable}.
Note that even though the only subtree with an edge to both $p_c$ and $p_2$ is $\tau_d$,
the path $p_2$ and subtrees connected to it are also in the component containing $p_c$.
Thus, the lowest edge on $p^*_{R'}$ may not always be from $\tau_d$.

\begin{remark}
%	Since the highest edge from the {\em eligible} subtrees on $path(r_c,r')$ is $(x_p,y_p)$,
	This traversal is not applicable only if there is an edge higher than $y_p$ on $path(r_c,r')$, 
	from $p_2$ or some subtree connected to $p_2$. % and not $p_c$.
\end{remark}







In this entire section $(x_p,y_p)$ and $(x_r,y_r)$ correspond to the  back edges used in 
$p$ and $r$ traversals described in Section~\ref{sec:heavyP}, where as 
$(x_{p'},y_{p'})$ and $(x_{r'},y_{r'})$ would correspond the  back edges used in modified $p'$
and $r'$ taversals described below. Our modified $p'$ traversal and $r'$ traversal would use 
$(x_{p'},y_{p'})=(x_3,y_3)$ and $(x_{r'},y_{r'})=(x_2,y_2)$ respectively, 
which will be followed by an appropriate traversal (see Figure \ref{fig:pdfsSp}).
We now recall the conditions leading to the {\em special} case its implications on
$(x_p,y_p)$, $(x_r,y_r)$ and $(x_d,y_d)$.

\begin{lemma}
	The conditions of the special case are (i) $x_3\in T(v_R)$, (ii) $x_p\in \tau_d$, and 
	(iii) $(x_r,y_r)=(x'_2,y'_2)$. Following are the properties of $(x_p,y_p)$ and $(x_d,y_d)$ 
	in this case.
	\begin{enumerate}
\item $y_d=y_p$,$y_3$ is lower than $y_d$ on $path(r_c,r')$, and $y_r$ is lower than $y_2$ on $path(r_c,r')$.
\item No subtree of $\tau_d$ hanging from $path(root(\tau_d),x_p)$, with an edge to $p_c$, 
		has an edge lower than $y_2$ on $path(r_c,r')$. %\label{obs:disconTd}
\item No subtree of $\tau_d$ hanging from $path(root(\tau_d),x_r)$, with an edge to $p_c$,
		has an edge higher than $y_3$ on $path(r_c,r')$. 	%\label{obs:disconTdx}
	\end{enumerate}			
	\label{lem:propSC}
\end{lemma}
\begin{proof}
Recall the choice of $(x_d,y_d)$ and $(x_p,y_p)$ (see Appendix~\ref{sec:choose_ep_ed}), it was the highest edge from 
$\tau_d$ on $path(r_c,r')$ and $(x_p,y_p)$ was computed such that $y_p\in path(y_d,r')$. 
Hence, if $x_p\in \tau_d$ we necessarily have $y_d=y_p$.
Also, $y_3$ is strictly lower than $y_p$ (or $y_d$) else having a lower $LCA(x_3,v_H)$ 
than $LCA(x_p,v_H)$, $(x_3,y_3)$ would have been selected as $(x_p,y_p)$ earlier.
Finally, $y_2$ is strictly higher than $y_r$ otherwise $(x_2,y_2)$ 
would have been selected as $(x_r,y_r)$ earlier.
Second property holds since $(x_2,y_2)$ (where $x_2\in T(v_P)$) was the lowest edge on $path(r_c,r')$
from the eligible subtrees after $p$ traversal. 
Third property holds since $(x_3,y_3)$ (where $x_3\in T(v_R)$) was the highest edge on $path(r_c,r')$
from the eligible subtrees after $r$ traversal.
\end{proof}



To handle this special case, we again check the scenario's corresponding to $p$ and $r$ traversals 
ignoring the {\em eligible} subtree $\tau_d$. Hence, the corresponding edges $(x_{p'},y_{p'})$ and $(x_{r'},y_r)$
for these scenarios does not emerge from $\tau_d$.  Thus, ignoring $\tau_d$, after each traversal 
the first two conditions of Lemma~\ref{lem:non-applicable} would be satisfied. In case this traversal can be 
followed by the traversal of $\tau_d$ such that Lemma~\ref{lem:non-applicable} is satisfied, 
it is performed else we move to the next traversal.

\subsection*{Modified {\large $p'$} traversal}
Consider a modified $p'$ traversal using $(x_{p'},y_{p'})=(x_3,y_3)$ instead of a higher $(x_p,y_p)$ 
as shown in Figure~\ref{fig:pdfsSp} (a), traversing the path 
$p^*_{P'}=path(r_c,x_3)\cup (x_3,y_3)\cup path(y_3,par(v_l))$ 
%T(see Figure~\ref{fig:pdfsSp} (a)). 
This leaves an un-traversed part of $path(r_c,r')$, say $p_1=path(par(y_3),r')$, 
that necessarily contains $y_d$ as $y_3$ is strictly lower than $y_d$ (see Lemma~\ref{lem:propSC}).
%This is because $y_3$ is strictly lower than $y_p$ (or $y_d$) else having a lower $LCA(x_3,v_H)$ 
%than $LCA(x_p,v_H)$, $(x_3,y_3)$ would have been selected as $(x_p,y_p)$ earlier.
Now, the computation of $(x_3,y_3)$ ensures that no {\em eligible} subtree (except for $\tau_d$)
is connected to both paths $p_1$ and $p_c$, as well as ensuring that $T(v_{P'})$ is not connected to $p_1$. 
This satisfies the first two conditions of Lemma~\ref{lem:non-applicable} ignoring $\tau_d$.
Since, $\tau_d$ is necessarily connected to two paths $p_1$ and $p_c$, its component will not be of 
type $C1$ or $C2$, which is not permissible.

%Thus, the subtree $\tau_d$ is connected to two paths $p_1$ and $p_c$, which is also the only subtree
%connected to both $p_1$ and $p_c$ (recall computation of $(x_3,y_3)$). 
%This is not permissible as the component having $\tau_d$ will not be of 
%type $C1$ or $C2$. 
%
%This is clearly not permissible as the component having $\tau_d$ and $p_c$ will not be of 
%type $C1$ or $C2$. 

However, if this traversal is followed by the traversal of $p_{P'}=(y_r,x_r)\cup (x_r,root(\tau_d))$
(see Figure~\ref{fig:pdfsSp} (a)), no subtree of $\tau_d$ connected to $p_c$ will be connected to 
$p_1$ (see property~3 in Lemma~\ref{lem:propSC}). 
This satisfies the first two conditions of Lemma~\ref{lem:non-applicable}.
Also, since $T(v_{P'})$ does not have an edge to $\tau_d$, after this traversal the component 
having $p_c$ would have the new root in $\tau_d$ or $p_c$, satisfying the third condition 
of Lemma~\ref{lem:non-applicable}. 
Thus, if the lowest edge on $p^*_{P'}$ from the component containing $p_c$ is from $\tau_d$,
i.e. $(x_r,y_r)$, the traversal of $p^*_{P'}$ followed by $p_{P'}$, 
satisfies Lemma~\ref{lem:non-applicable}. 
Note that even though the only subtree with an edge to both $p_c$ and $p_1$ is $\tau_d$,
the path $p_1$ and subtrees connected to it are also in the component containing $p_c$.
Thus, the lowest edge on $p^*_{P'}$ may not always be from $\tau_d$.

\begin{remark}
%Since the lowest edge from the {\em eligible} subtrees on $path(r_c,r')$ is $(x_r,y_r)=(x'_2,y'_2)$,
	This traversal is not applicable only if there is an edge lower than $y_r$ on $path(r_c,r')$, 
	from $p_1$ or some subtree connected to $p_1$.
	% (not directly to $p_c$).
\end{remark}

\subsection*{Modified {\large $r'$} traversal}
Consider a modified $r'$ traversal using $(x_{r'},y_{r'})=(x_2,y_2)$ instead of a lower $(x_r,y_r)$
traversing the path $p^*_{R'}=path(r_c,x_{r'})\cup (x_{r'},y_{r'})\cup path(y_{r'},r')$ 
(see Figure~\ref{fig:pdfsSp} (b)). 
This leaves an un-traversed part of $path(r_c,r')$, say $p_2=path(par(v_l),y_2)\backslash\{y_2\}$,
that necessarily contains $y_r$ 
as $y_2$ is strictly higher than $y_r$ (see Lemma~\ref{lem:propSC}).
%. This is because $y_2$ is strictly higher than $y_r$
%otherwise $(x_2,y_2)$ would have been selected as $(x_r,y_r)$ earlier.
Now, the computation of $(x_2,y_2)$ ensures that no {\em eligible} subtree (except for $\tau_d$)
is connected to both paths $p_2$ and $p_c$, as well as ensuring that $T(v_{R'})$ is not connected to $p_2$. 
This satisfies the first two conditions of Lemma~\ref{lem:non-applicable} ignoring $\tau_d$.
Since, $\tau_d$ is necessarily connected to two paths $p_2$ and $p_c$, its component will not be of 
type $C1$ or $C2$, which is not permissible.
%Thus, the subtree $\tau_d$ is connected to two paths $p_2$ and $p_c$, which is also the only subtree
%connected to both $p_2$ and $p_c$ (recall computation of $(x_2,y_2)$). 
%This is not permissible as the component having $\tau_d$ will not be of 
%type $C1$ or $C2$. 
%%This is clearly not permissible as the component having $\tau_d$ and $p_c$ will not be of 
%%type $C1$ or $C2$. 

However, if this traversal is followed by the traversal of $p_{R'}=(y_p,x_p)\cup (x_p,root(\tau_d))$
(see Figure~\ref{fig:pdfsSp} (b)), no subtree of $\tau_d$ connected to $p_c$ will be connected to 
$p_2$ (see property~2 in Lemma~\ref{lem:propSC}). 
This satisfies the first two conditions of Lemma~\ref{lem:non-applicable}.
Also, since $T(v_{R'})$ does not have an edge to $\tau_d$, after this traversal the component 
having $p_c$ would have the new root in $\tau_d$ or $p_c$, satisfying the third condition 
of Lemma~\ref{lem:non-applicable}. 
%Also, since $\tau_d$ is connected to $p_c$, after this traversal the component 
%having $p_c$ would have the new root in $\tau_d$, satisfying the third condition 
%of Lemma~\ref{lem:non-applicable}. 
Thus, if the lowest edge on $p^*_{R'}$ from the component containing $p_c$ 
is from $\tau_d$, i.e. $(x_p,y_p)$, the traversal of $p^*_{R'}$ followed by $p_{R'}$, 
satisfies Lemma~\ref{lem:non-applicable}.
Note that even though the only subtree with an edge to both $p_c$ and $p_2$ is $\tau_d$,
the path $p_2$ and subtrees connected to it are also in the component containing $p_c$.
Thus, the lowest edge on $p^*_{R'}$ may not always be from $\tau_d$.

\begin{remark}
%	Since the highest edge from the {\em eligible} subtrees on $path(r_c,r')$ is $(x_p,y_p)$,
	This traversal is not applicable only if there is an edge higher than $y_p$ on $path(r_c,r')$, 
	from $p_2$ or some subtree connected to $p_2$. % and not $p_c$.
\end{remark}

\subsection*{Residual {\large $r''$} traversal}
The remarks of modified $p'$ traversal and modified $r'$ traversal shows that 
$path(par(v_l),y_r)\backslash\{y_r\}$ (say $p_3$) and $path(par(y_p),r')$ (say $p_4$)
are connected either directly by an edge or some subtree $\tau'$ having edge to both $p_3$ and $p_4$ 
and not to $p_c$ (see Figure~\ref{fig:pdfsSp} (c)). Let the lowest such edge on $p_3$ be 
$(x',y')$ (if directly connected) or $(y_{\tau'},y')$ (if connected via $\tau'$) 
where $y'\in p_3$. In the latter case let the highest edge from $\tau'$ on $p_4$ 
be $(x',x_{\tau'})$.  
In both cases, we call this path from $x'$ to $y'$ as $p_{\tau'}$, i.e.,
$p_{\tau'}=(x',y')$ or $p_{\tau'}=(x',x_{\tau'})\cup path(x_{\tau'},y_{\tau'})\cup (y_{\tau'},y')$.

We then perform the traversal shown in Figure~\ref{fig:pdfsSp} (c), where 
$p^*_{R''}=path(r_c,x_2)\cup (x_2,y_2)\cup path(y_2,x')\cup p_{\tau'}\cup path(y',y_2)\backslash\{y_2\}$.
As a result, we have three unvisited paths, $p_c$, 
$p'=path(par(x'),r')$ (say $p'_4$) and 
$p''=path(par(v_l),y')\backslash\{y'\}$ (say $p'_3$).
Now, the unvisited part of $\tau'$ is not connected to $p_c$ (see remark in $p'$ and $r'$ traversal) and 
$p'_3$ or $p'_4$ (by construction) which forms a separate component. 
Also, any subtree connected to $p'_4$ is not connected to $p'_3$ ($y'$ is the lowest edge on $p_2$). 
Further, subtree $\tau_d$ (and hence any subtree connected to $p_c$) is not connected to $p'_3$ or $p'_4$ 
(as $y_r\notin p'_3$ and $y_p\notin p'_4$).
Finally, the component having path $p_c$ will have the lowest edge to $p^*_{R'}$
in $\tau_d$, which is not a heavy subtree. Hence, the traversal of $p^*_{R''}$ 
satisfies the conditions of Lemma~\ref{lem:non-applicable}.
Refer to Procedure~\ref{alg:dfs_c2sp} in Appendix~\ref{appn:pseudocode} for the pseudo code.


==> heavySubAlt.tex <==
\subsubsection{Heavy Subtree Traversal}
Consider a component $c$ of type $C2$, where $r_c\in\tau$ where  $\tau \in \TT_c$ and $r'$ is the root of $\tau$.
As described earlier, if $r_c$ is the root of $\tau$ or $r_c\in T(v_H)$ it can be processed using 
disintegrating or disconnecting traversals respectively. 
Otherwise, we traverse the heavy subtree $\tau$ using a combination of disintegrating and disconnecting traversals
such that every unvisited component of $c$ can be moved to the next phase.

We first perform a disintegrating traversal of $\tau$ (despite $c$ being of type $C2$), 
which leads to formation of another path, i.e., the unvisited part of $path(r_c,r')$ 
in addition to the path $p_c$ in the component.
Hence, the newly formed component is neither of type $C1$ nor $C2$. 
Thus, the aim of the remainder of this traversal is to make sure $p_c$ is completely traversed
so that the components of the unvisited part of $c$ are of types $C1$ and $C2$ in the next phase.
For this purpose we relax the requirement for $c$ to be of type $C1$ and $C2$ only, during
the remainder of the phase. During this period the component $c$ is of the following type.

\begin{itemize}
\item[C3:] Consists of a single {\em ancestor-descendant} path $p_c$ called as the {\em primary} path 
			and a set $P_c$  of  {\em ancestor-descendant} paths called as the {\em secondary} paths.
			Moreover, we have a set ${\cal T}_c$ of subtrees of the DFS tree $T$ having at least one edge to $p_c$ or $P_c$. 
			Each subtree in $\TT_c$ is connected to at most one secondary path. 
			Let $\TT_{c_k}$ denote the set of subtrees in $\TT_c$ connected to secondary path $p_k\in P_c$.
			Also $\TT_{c_0}$ denotes the subtrees having an edge only to $p_c$ and not to any $p_k\in P_c$. 
\end{itemize}

Again, for every component $c$ we also have a vertex $r_c\in c$ from which the DFS tree of the component $c$ 
would be rooted in the final DFS tree $T^*$. However, for a component $c$ of type $C3$, even if 
$|\tau_c|\leq n_0/2^i$ we do not move it to the next phase. But we shall move $c$ to the next stage 
based on size of $p_c$ as described earlier.

Now, as described earlier heavy path traversal of $\tau\in \TT_c$ creates a secondary path $p_k$ 
and all the unvisited subtrees of $\tau$ are added to $\TT_{c_k}$. However, since disintegrating traversal
was performed on $\tau$, we know that $|\tau|\leq n_0/2^i$.
If the resultant $r_c$ belongs to either $p_c$ or $\TT_{c_0}$ it is processed similar to 
components of type $C2$, i.e., path halving for $r_c\in p_c$, disconnecting traversal if $r_c\in \TT_{c_0}$ and $r_c\notin \Th_c$ 
and disintegrating traversal if $r_c\in \TT_{c_0}$ and $r_c\in \Th_c$. 
Thus, any subtree $\tau$ in $\TT_{c_k}$, for $k\neq 0$ will surely satisfy $|\tau|\leq n_0/2^i$.
Hence, when $p_c$ is completely traversed all the resulting components containing secondary paths can be moved
to the next phase as components of type $C2$. Components having no secondary paths will be converted to type $C1$
and processed in the final stage of the phase.

We now describe how to process the component if $r_c \in \TT_{c_k}$, for $k\neq 0$ or $r_c\in p_k$.
In order to move to the next stage our traversal needs to reach $p_c$. 
This can be achieved in $O(\log n)$ steps, where in each step we perform disconnecting traversal 
followed by path halving. 
However, if $r_c\in p_k$, we directly perform path halving of $p_k$. 
Thus, in $O(\log n)$ steps either $p_k$ would be completely
traversed or the traversal would have reached $p_c$ ending the stage. 


Now, if $r_c\in \tau \in \TT_{c_k}$ ($k\neq 0$), we perform the disconnecting traversal of $\tau$ 
from $p_k$ (not from $p_c$) as follows. This is performed similar to one described in Section \ref{sec:discon}
except that instead of $p_c$, we choose to disconnect the resulting components from $p_k$.
Recall that disconnecting traversal of $\tau$ from a path $p$ ($p_c$ in Section \ref{sec:discon}, here $p_k$) 
traverses $\tau$ to reach $p$ (say at $v\in p$) followed by path halving of $p$ such that the
remaining part of $p$ (say $p'$) is not connected to the unvisited part of $\tau$. 
This creates a new path $p_{k'}$ from $\tau$ having the unvisited part of $path(r_c,r')$. 
The subtrees in the unvisited part of $\tau$ connected to $p_{k'}$ would then be added to $\TT_{k'}$.
The remaining subtrees will not have any secondary path. as their secondary path if they are connected to it. 

However, in case the lowest edge  on traversed part of $p_k$ (and hence resultant $r_c$) belong to $p_{k'}\cup \TT_{k'}$
we cannot ensure the progress of this step. This is because the new secondary path is $p_{k'}$ which can be of arbitrary length.
In such a case we would perform 
 
Now, after disconnecting traversal and the corresponding path halving 
let the lowest edge on traversed part of $p_k$ by $(x,y)$, where $x\in \tau$ and $y\in p_k$.
Clearly, the new root of the unvisited part of $c$ would be $x$. 
Now, based on the location of $x$ we can have three cases.
\textit{Firstly}, if $x\in p_c$, the traversal has simply reached $p_c$ in a single step ending the stage. 
\textit{Secondly}, if $x\in p_k\cup \TT_{c_k}$, we have proceeded to the next step as size of secondary path $p_k$ is halved.
However, in the third case where $x\in p_{k'} \cup \TT_{c_{k'}}$, we cannot ensure the progress of this step. 
This is because the new secondary path is $p_{k'}$ which can be of arbitrary length.
In such a case we do not perform the previous disconnecting traversal of $\tau$, 
rather we traverse $\tau$ along $path(r_c,x)$ to reach $p_k$ at $y$ and then traverse $p_k$ towards $v$ (where traversal was supposed to enter $p_k$).
This ensures that the unvisited part of $p_k$ is neither connected to $p_c$ nor to any other subtree 
(as $(x,y)$ was the lowest edge on orignally traversed
The path can then be traversed independent of the other components attaching it directly to $y$.
This also ends the step 
Thus, in a heavy subtree traversal each stage can be completed in $O(\log n)$ steps.

==> pdfs2.tex <==
% NOTATAIONS:::
% \tau_c heaviest tree of the component c
% p_c  path of the component c
% T(v_H) Smallest subtree with size > n_0/2^i


\section{Rerooting a DFS tree}
\label{sec:pdfs}
%%%%% UPDATE DS QUERY SYNTAX IN PSEUDOCODE
%%%% FIGURE FOR C1 and C2P2
%%%%% Remark for O(\log^2 n) using m processors
We now describe an algorithm to reroot a subtree  $T(r_0)$ of the DFS tree $T$, 
from its original root $r_0$ to the new root $r^*$. Let the number of vertices and edges of the subgraph induced by
$T(r_0)$ be $n_0$ and $m_0$ respectively. 
Given the current DFS tree $T$ of the graph and data structure $\cal D$ built on it, 
the following algorithm requires $n_0$ processors 
to perform this rerooting in $O(\log^3 n)$ time on EREW PRAM. 
The algorithm is divided into $\lfloor\log n_0\rfloor$ {\em phases}, where each phase is further divided 
into $\lfloor\log n_0\rfloor$ {\em stages}.
For notational convenience, we refer to the phases as $P_0,P_1.P_2,...$ and the stages during a phase
as $S_0,S_1,S_2,...$ . Furthermore, at the beginning of every phase and every stage, the structure of 
every component $c$ of the unvisited graph can be of the following types:

\begin{itemize}
\item[C1: ] The component would be a single subtree $\tau_c$ of the DFS tree $T$. We would also have a vertex $r_c\in \tau_c$
			from which the DFS tree of the component $c$ would be rooted in the final DFS tree $T^*$.
\item[C2: ] The component would have a single {\em ancestor-descendant} path $p_c$ and a set 
			${\cal T}_c$ of subtrees of the DFS tree $T$. We would also have a vertex $r_c\in {\cal T}_c\cup p_c$ from which
			the DFS tree of the component $c$ would be rooted in the final DFS tree $T^*$. 
			Note that for any $\tau_1,\tau_2\in{\cal T}_c$, there is no edge between $\tau_1$ and $\tau_2$ since $T$ is a DFS tree.
\end{itemize}

At the beginning the phase $P_i$ of the algorithm, every subtree of each component $c$ ($\tau_c$ or subtrees in ${\cal T}_c$)
would have at most $n_0/2^i$ vertices. Note that during the phase $P_i$, every component can have exactly one heavy subtree
with more than $n_0/2^{i+1}$ vertices. If no such tree exists we move the component $c$ to the next phase.
Further, in case the component is of type $C1$, the heavy subtree would be $\tau_c$. For notational convenience, we refer the heavy subtree of
every component $c$ as $\tau_c$ (even for components of type $C2$). Clearly the algorithm ends after $O(\log n_0)$ phases as every 
component of the unvisited graph would be empty.  

At the beginning of the stage $S_j$ of a phase, length of the path $p_c$ in each component $c$ would be at most
 $n_0/2^j$. If $|p_c|\leq n_0/2^{j+1}$, we move the component $c$ to the next stage.
Note that in case the component $c$ is of type $C1$, the value of $|p_c|$ is zero, so we move such components to the last stage of the phase i.e. $S_{\log n_0}$. Clearly each phase shall end after $O(\log n_0)$ stages.

The algorithm begins in the final stage $S_{\log n_0}$ of the first phase $P_0$, 
where the component induced by $T(r_0)$ is of type $C1$ and $r_c=r^*$. 
Note that during each stage, different connected components of the unvisited graph can be 
processed independent of each other in parallel. The number of processors assigned to each component is 
equal to the number of vertices in the component. 
% Thus, if each stage of the algorithm can be completed in $t$
% time, the total time taken by the algorithm is $O(t \log^2 n_0)$.
 

\subsection{A phase of the algorithm}
We shall now describe how a component $c$ is processed when it enters a phase $P_i$.
The aim of each phase is to build a partial DFS tree for the component $c$ rooted at $r_c$ 
that can be attached to the already build DFS tree $T^*$ of the updated graph.
However, we need to ensure that at the end of the phase the components of the 
unvisited part of $c$ can be moved to the next phase, 
i.e. each component $c'$ is of type C1 or C2 with $|\tau_{c'}|\leq n_0 / 2^{i+1}$.
Let the smallest subtree of $\tau_c$ that have at least $|\tau_c|/2$ vertices be $T(v_H)$.
Thus, at the end of the phase we need to ensure that some part of $T(v_H)$ is traversed 
dividing it into smaller subtrees. 
%This is achieved by guiding the DFS traversal in such a way that the unvisited part of
%$c$ is divided into different components each having the heavy subtree
%of size at most $n_0/2^{i+1}$. 
This can be achieved in $\log n_0$ stages as described in the 
following section.


\subsection{A stage of the algorithm}
We shall now describe how a component $c$ is processed when it enters a stage $S_j$
based on the type of the component. 
%The correctness of each stage of the algorithm 
%requires the components property to be satisfied for the newly added part of the tree $T^*$.

\begin{figure}[!hb]
\centering
\includegraphics[width=.75\linewidth]{Figures/pdfs_eg1.pdf}
\caption{The three types of traversals (blue dotted lines) for (a) Component $C1$, 
(b) Component $C2$ Part 3 and (c) Component $C2$ Part 2.}
\label{fig:pdfs1}
\end{figure}



\subsubsection{Component type 1}
\label{sec:c1}
%%%%%% OR SIMPLY EXTRACT PATH $V_H$ to $R'$ and convert to $C2$

Consider a component $c$ of type $C1$ in phase $P_i$. 
As described above, this component is moved to stage $S_{\log {n_0}}$. 
The component $c$ is the subgraph induced by a single subtree $\tau_c$ 
of the original DFS tree $T$ such that $n_0/2^{i+1} \leq |\tau_c| < n_0/2^i$. 
We are required to perform the DFS traversal of this subgraph
from the vertex $r_c\in \tau_c$ such that each component $c'$ of the unvisited part of $c$ 
is of type $C1$ or $C2$ with $|\tau_{c'}|\leq |\tau_c|/2$. 
We find the smallest subtree of $\tau_c$ having $|\tau_c|/2$ vertices i.e. $T(v_H)$.

We want the traversal to go from $r_c$ towards $v_H$ such that all the subtrees 
eventually hanging from this path have size less than $|\tau_c|/2$.
Also, we need to make sure that the components of the unvisited part of $\tau_c$ are of types
$C1$ or $C2$. 
This can be achieved by traversing along the tree path $path(r_c,v_H)$  and adding it to $T^*$. 
Let the subtree hanging from $path(r_c,root(\tau_c))$ containing $v_H$ be $T(v_h)$.

%
%We want the traversal to go from $r_c$ towards $v_H$ such that all the subtrees 
%eventually hanging from this path have size less than $|\tau_c|/2$.
%%Also, we need to make sure that the components of the unvisited part of $\tau_c$ are of types
%%$C1$ or $C2$. 
%This can be achieved by traversing along the tree path connecting $r_c$ and $v_H$. i.e. 
%$path(r_c,v_l)\cup path(v_l,v_H)$ and adding it to $T^*$, where $v_l=LCA(r_c,v_H)$.
%%Let the subtree hanging from $path(r_c,root(\tau_c))$ containing $v_H$ be $T(v_h)$.
%
%Now, the unvisited part of $c$ consists of a path $p\leftarrow path(par(v_l),root(r_c))$ and
%the subtrees hanging from $path(r_c,v_l)\cup path(v_l,v_H)$
%
%the remaining 
%the path unvisited part of $path(r_c,root(\tau_c))$ 
%(say $p$, which is an ancestor-descendant path of $T$) 
%and the subtrees hanging from the $path(r_c,root(\tau_c))$ and $path(v_h,v_H)$ 
%each having size less than $|\tau_c|/2$. 
%Each subtree not having an edge to $p$ corresponds to a separate 
%connected component of type $C1$. The path $p$ and the remaining subtrees 
%(having an edge to $p$) forms a component of type $C2$. 
%Thus, all these components can be moved to the next phase.
%
%
%
%%Collect the set of subtrees hanging from this path in $\cal T$. 

Now, the unvisited part of $c$ consists of the remaining 
unvisited part of $path(r_c,root(\tau_c))$ 
(say $p$, which is an ancestor-descendant path of $T$) 
and the subtrees hanging from the $path(r_c,root(\tau_c))$ and $path(v_h,v_H)$ 
each having size less than $|\tau_c|/2$. 
Each subtree not having an edge to $p$ corresponds to a separate 
connected component of type $C1$. The path $p$ and the remaining subtrees 
(having an edge to $p$) forms a component of type $C2$. 
Thus, all these components can be moved to the next phase.

Now, for each component $c^*$ moved to the next phase we also need to find 
the new root $r_{c^*}$ for the DFS tree of the component.
Using the components property we know this is the lowest edge from $c^*$ the path $p^*$ attached to $T^*$. 
This added path $p^*$ is $path(r_c,par(v_h))$ followed by $path(v_h,v_H)$. 
We query our data structure $\cal D$ to find the lowest edge from each subtree and path in $c^*$ to $p^*$.  
The end point of this edge in $c^*$ is the new root $r_{c^*}$ for the DFS tree of $c^*$.
Refer to Procedure \ref{alg:dfs_c1} in Appendix \ref{appn:pseudocode} for the pseudo code for a stage for components of type $C1$.


%% Write Independently
%% Input, Output(Component of type 2 in next phase), Time analysis, Space required.
%% Model Required EREW or CRCW? If not reason or specific areas which cause this. 
%% Keep in mind the Distributed setting as well.
\subsubsection{Component type 2}


Consider a component $c$ of type $C2$ in phase $P_i$ and stage $S_j$. 
Thus, $c$ is the subgraph induced by an ancestor-descendant path $p_c$ and 
some subtrees of $T$ with the heaviest subtree $\tau_c$ such that 
$n_0/2^{j+1} \leq |p_c| < n_0/2^j$ and $n_0/2^{i+1} \leq |\tau_c| < n_0/2^i$.
We are required to perform the DFS traversal of this subgraph
from the vertex $r_c$ in $\tau_c$ such that each component $c'$ of the unvisited part of $c$ 
either has  $|\tau_{c'}|\leq |\tau_c|/2$ (moving to the next phase) or $|p_{c'}|\leq |p_c|/2$ (moving to the next stage). 


Now, we shall describe the three parts in which this stage is completed.
However, in order to explain the intuition behind the approach we shall describe these parts in the 
reverse chronological order. A component can also start directly in the second or third part
as described below.

\begin{itemize}
\item \textbf{Part 3:} When $r_c \in p_c$ or $r_c\in T(v_H)$: 

In case $r_c\in p_c$, we traverse $p_c$ from $r_c$ to the farther end of (say $x$), 
reducing $p_c$ to half of its original length. Hence, we add $path(r_c,x)$ to the tree $T^*$.
Now, the unvisited part of $c$ consists of the remaining unvisited part of $p_c$ 
and the subtrees of $c$. 

In case $r_c\in T(v_H)$, we traverse from $r_c$ to the root of $\tau_c$, adding $path(r_c,root(\tau_c))$ to $T^*$.
Since, $r_c\in T(v_H)$ all the subtrees hanging from $path(r_c,root(\tau_c))$ have size at most half of $|\tau_c|$.
In addition to these subtrees, the unvisited part of $c$ consists of the path $p_c$ and the other subtrees in $\TT_c\setminus \tau_c$. 

The subtrees not having an edge to the final $p_c$ (having edges only on $path(r_c,x)$ if $r_c\in p_c$ or $path(r_c,root(\tau_c))$ otherwise) 
corresponds to separate connected components of type $C1$ and can be moved to the appropriate phase and 
stage accordingly. 
The path $p_c$ and the remaining subtrees (having an edge to $p_c$) form a component of type $C2$. 
The component $c$ can be moved to the next stage (if originally $r_c\in p_c$, as $p_c$ reduced to half) or 
the next phase (if originally $r_c\in T(v_H)$, as $|\tau_c|$ reduced to half). 
The new root for each component can be found similar to what is described in Section \ref{sec:c1}.
Refer to Procedure \ref{alg:dfs_c2_3} in Appendix \ref{appn:pseudocode} for the pseudo code of this part of the algorithm.\\

%Clearly, the components property is satisfied in the algorithm by construction,
%ensuring the correctness of this algorithm.
%Also, in Procedure \ref{alg:dfs_c1} each line (except the queries to data structure $\cal D$)
%can be performed in $O(1)$ time using $|c|$ processors in parallel. 
%The data structure queries require $O(\log n)$ for querying a subtree $\tau$ using $|\tau|$ processors, 
%requiring overall $c$ processors in parallel.
%Thus, we have the following:
%
%\begin{theorem}
%	For a component $c$ of type $C2$, a stage can be completed in $O(\log n)$ time 
%	using $|c|$ processors in CRCW PRAM model. 
%\end{theorem}
%Figure



\item \textbf{Part 2:} When $r_c \in \tau\neq \tau_c$ or $r_c\in T(v_H)$:

%In case this assumption does not hold, we have $r_c\in \tau \neq \tau_c$. 
We shall start the traversal from $r_c$ through $\tau$ to reach $p_c$ and then move to the third part
of the stage. However, this shall be performed making sure that the unvisited part of $\tau$ 
is not connected to the remaining unvisited part of $p_c$ (say $p'$). Also, the components of 
the unvisited part of $\tau$ should be of type $C1$ or $C2$ only. 
This makes the unvisited part of $\tau$ independent of $p'$, 
moving its components to the next phase (as they are no longer connected to $\tau_c$).
Hence, we call this traversal a {\em disconnecting} traversal as it disconnects the 
unvisited components of $\tau$ from $p_c$.


Suppose we enter $p_c$ such that all edges from $\tau$ on $p_c$ are on the longer side of the divided $p_c$.
This would ensure that $\tau$ is disconnected from $p'$ as all edges from $\tau$ would be on the visited part of $p_c$.
Hence, we first find the lowest edge from $\tau$ to the path $p_c$ 
(say $(x,y)$, where $y\in p_c$ and $x\in \tau$).
However, if $x$ is higher than the midpoint of $p_c$, the traversal would follow to the lower end of $p_c$.
In that case, we find the highest edge from $\tau$ to the path $p_c$ so that it surely traverses 
to the lower end of $p_c$ on entering it (highest edge is surely on upper half of $p_c$ as lowest edge was on upper half of $p_c$). Again, let $(x,y)$ be this edge, where $y\in p_c$ and $x\in \tau$. 
To complete the description we now have to describe how 
to traverse through $\tau$ to reach $x$. This can be done by traversing through the tree path
i.e. from $r_c$ to $x$ through $LCA(r_c,x)$. Hence, we add $path(r_c,x)$ to the DFS tree $T^*$.
Let the subtree hanging from $path(r_c,root(\tau))$
containing $x$ be $T(v)$.

Now, the unvisited part of $\tau$ consists of the remaining unvisited part of $path(r_c,root(\tau))$ 
(say $p$, which is an ancestor-descendant path of $T$) and the subtrees hanging from the $path(r_c,root(\tau))$ 
(except $T(v)$) and $path(v,x)$. Since no subtree has any edge to $p'$, the subtrees not having an edge to $p$ 
corresponds to a separate connected components of type $C1$. The path $p$ and the remaining subtrees 
(having an edge to $p$) forms a component of type $C2$. Thus, all these components can be moved to the next phase.
The new root for each component can be found as described in Section \ref{sec:c1}.
Refer to Procedure \ref{alg:dfs_c2_2} in Appendix \ref{appn:pseudocode} for the pseudo code of this part of the algorithm.



%\end{proof}


\begin{figure}[!hb]
\centering
\includegraphics[width=\linewidth]{Figures/pdfs_eg.pdf}
\caption{The three types of traversals (blue dotted lines) in Part $1$ of component $C2$.}
\label{fig:pdfs}
\end{figure}


\item \textbf{Part 1:} When $r_c \in \tau_c$:

Note that the {\em disconnecting} traversal cannot be performed in $\tau_c$ 
as in the resulting component $c'$ disconnected from $p_c$ can have a heavy subtree 
(more than $n_0/2^{i+1}$ vertices) with the new path $p_{c'}$ of arbitrary large length
(as compared to $p_c$).
We now present a few notations that shall be used in the rest of the section to denote some parts of 
$\tau_c$. Let $r'$ be the root of $\tau_c$, and $T(v_h)$ be the heaviest subtree hanging from $path(r_c,r')$.

This part is performed in three steps. In each step, the traversal would follow the path as described 
in Figure \ref{fig:pdfs} in certain cases, in the other cases it would move to the next step.\\

%\begin{case}
%Highest edge on $r_c$ to $r'$ from subtrees hanging on the $path(r_c,r')$.
%Follow the path from $r_c$ to $r'$ 
%\end{case}
%Prob: Lowest edge $(x,y)$ in $T(v_h)$.

\begin{step}
	\textbf{Traversal of the form Figure \ref{fig:pdfs} (a).}
\end{step}
We first find the highest edge on $path(r_c,r')$ from subtrees hanging from it (except $T(v_h)$)
and subtrees hanging from $path(v_h,v_H)$. We consider only those subtrees that have an edge to $p_c$.
Let this edge be $(x,y)$, where $y\in path(r_c,r')$. We store this edge as $(x^*,y^*)$ to be used in the last step.
Now, we have two cases before we move to the next step.

In case $x\notin T(v_h)$, we perform another check before making a {\em disconnecting} traversal 
through it to halve $p_c$, ending the stage (see Figure \ref{fig:pdfs}(a)).
Firstly, if $T(v_h)$ does not have an edge to $p_c$, we simply add $path(r_c,r')$ and edge $(x,y)$
to $T^*$ moving to part two, with new root $x$. This ensures that new $\tau_c$ would move to the 
final stage of the phase.
Otherwise, We find the highest edge on $path(r_c,r')$ from subtrees hanging from $path(v_h,v_H)$ without 
having an edge to $p_c$. 
If no such edge exist we find such an edge from entire $T(v_h)$
(this might be possible if edge is on $path(v_h,v_H)$). In case we find such an edge, we call it $(x,y)$
and move to next step.

Now, if $x\in T(v_H)$ or we did not find the edge as described above, we perform a 
{\em disconnecting} traversal through the edge (as shown in Figure \ref{fig:pdfs}(a)).
by adding $path(r_c,y)$ to the tree $T^*$ and leaving through $(y,x)$ in part 2.
Note that this may leave an unvisited path $path(par(y,r')$, which however is not 
connected to any subtree first queried during this step. Hence, it is not connected to $p_c$
and the corresponding component can be moved to the next phase with $r_c=par(y)$.

Hence, for the next step we have an edge $(x,y)$ from $T(v_h)$ to $path(r_c,r')$.\\

\begin{step}
	\textbf{Traversal of the form Figure \ref{fig:pdfs} (b).}
\end{step}
Let $T(v_{h_1})$ be the subtree hanging from $path(v_h,x)$ that contains $T(v_H)$.
Find the lowest edge from the subtrees hanging from $path(r_c,r')$ (except $T(v_h)$)
and $path(v_h,x)$ tp $path(y,par(v_h))$. Let this edge be $(x_1,y_1)$.

Now, if $x\in T(v_H)$ or $x\notin T(v_{h_1})$, we perform a 
{\em disconnecting} traversal through the edge (as shown in Figure \ref{fig:pdfs}(b))
by adding $path(r_c,x)\cup path(y,par(v_h))$ to the tree $T^*$ and leaving through $(y_1,x_1)$
in part 2.
Note that this may leave an unvisited path $path(par(y),r')$, which however is not 
connected to any subtree first queried during this step. Hence, it is not connected to $p_c$
and the corresponding component can be moved to the next phase with $r_c$ given 
by lowest edge from the component on $path(y,r_c)$.

Otherwise, we move to the next step, where we have two edges $(x,y)$ and $(x_1,y_1)$
from $T(v_h)$ to $path(r_c,r')$ such that $x_1\in T(v_{h_1})$.\\

\begin{step}
	\textbf{Traversal of the form Figure \ref{fig:pdfs} (c).}
\end{step}
We shall now use the edge $(x^*,y^*)$ stored in the first step to perform traversal as follows.
We follow the path $path(r_c,x_1)$ then using $(x_1,y_1)$ to enter $path(y_1,r')$ and later exit through $(x^*,y^*)$.
Now, in order to prove that this path indeed satisfies the components property consider the following arguments.
Recall the query for finding $(x^*,y^*)$, let the subtree containing $x^*$ in the first query be $\tau$.
If $x^*\in T(v_h)$ then it does not lie on $path(v_h,v_H)$.
Now, as $x_1$ belonged to $T(v_{h_1})$, $path(v_h,x_1)$ would follow $path(v_h,v_H)$ at least till $root(\tau)$.
Thus, $\tau$ would still be the highest subtree with an edge to $p_c$ on the path as shown in Figure\ref{fig:pdfs} (c).
If $x^*\notin T(v_h)$, then no subtree on $path(v_h,x_1)$ having edge to $p_c$ can have and edge higher 
than $\tau$ on $path(r_c,r')$, otherwise $\tau$ would not have the highest edge back then.
Refer to Procedure \ref{alg:dfs_c2} in Appendix \ref{appn:pseudocode} for the pseudo code of this part of the algorithm.


\end{itemize}

\subsubsection*{Correctness:}
To prove the correctness of the algorithm we need to ensure that the components
property is satisfied by each stage, part and step of the algorithm.
We also need to ensure that every component in a phase/stage, abides by the size constraints defining the phase/stage.
By construction we always choose the lowest edge from a component to the recently
added path in $T^*$ ensuring that the components property is satisfied.
Furthermore, the different parts and steps of the algorithm also ensures the size constraints of a phase/stage by construction.
Thus, the final tree $T^*$ returned by the algorithm is indeed the 
DFS tree of the updated graph.

\subsubsection*{Analysis:}
We now analyze the time required by each stage of the algorithm. 
Every instruction of the algorithm (refer to Appendix \ref{appn:pseudocode} for the pseudo code)
except for data structure queries and finding highest/lowest edge, 
can be performed in $O(1)$ time using $|c|$ processors (using Theorem \ref{thm:DSx})
The data structure queries of the type $Query(T(w),path(x,y))$ require $O(\log n)$ time 
using $|T(w)|$ processors (using Theorem \ref{thm:DS}), 
requiring overall $c$ processors. 
The data structure queries of the type $Query(path(u,v),path(x,y))$ require $O(\log n)$ time 
 using $\max(|path(v,w)|,|path(x,y)|)$ processors (using Theorem \ref{thm:DS}). 
 However, since each set of parallel data structure
 queries include at most one path query ($p_c$ for a component $c$), the overall $c$ processors 
 would suffice to perform these queries. 
Also the minimum/maximum of a set of numbers and hence the lowest/highest edge from a set of edges can be computed in $O(\log n)$ time
using $n$ processors (refer to Theorem \ref{thm:sort} in Appendix \ref{sec:ds}). 
Thus, each stage is completed in $O(\log n)$ time using $n$ processors. 
Since our algorithm completes in $\log n$ phases each requiring $O(\log n)$ stages we have the following theorem.

\begin{theorem}
	Given an undirected graph with the data structure $\cal D$ build on its DFS tree, for any given update in the graph
	the updated DFS tree can be computed in $O(\log^3 n)$ time using $n$ processors in EREW PRAM model. 
	\label{thm:reroot}
\end{theorem}

Thus, we can use Theorem \ref{thm:DS} and Theorem \ref{thm:reroot} to prove our main result in Theorem \ref{main-result}.

%\subsubsection{Rest}
%% Overall statement of a phase with time, space and dependence (EREW/CRCW)
%% Overall statement of Reroot and hence dynamic DFS, time, space, proc, EREW/CRCW.
%% Keep in mind the Distributed setting as well.

\subsection{Converting to Parallel Fully Dynamic DFS}
Firstly, we need to build the DFS tree of the original graph. 
This can be build using the static DFS algorithm \cite{Tarjan72} 
or any advanced parallel algorithm \cite{GoldbergPV88,AggarwalA88}.
Now, whenever the graph is updated we first build the data structure $\cal D$ 
on the existing DFS tree in $O(\log n)$ time using $O(m)$ processors (Theorem \ref{thm:DS}). 
We then convert the graph update into appropriate rerooting procedure computing the
final DFS tree in $O(\log^3 n)$ time using $O(n)$ processors (Theorem \ref{thm:reroot}).
We can similarly process any future updates using the current DFS tree.
Thus, we have the following theorem

\begin{theorem}
	Given any arbitrary online sequence of vertex or edge updates, 
	we can maintain a DFS tree in $O(\log^3 n)$ time per update 
	using $m$ processors in parallel EREW model.
\end{theorem}

%%\noindent BUILDING LCA STRUCTURE NOT SUPPORTED IN O(1) time
%%\textbf{Note: } The cost of answering data structure queries adds a $O(\log n)$ factor to the update time.
%% In CRCW model, the LCA queries are answerable in $O(1)$ time, whereas queries on $\cal D$ can be performed 
%% in $O(1)$ time by using $m$ processors in priority CRCW model replacing the binary search (see Appendix \ref{sec:ds}). Thus, the result can be improved to $O(\log^2 n)$ time per update using $m$ processors in a CRCW PRAM. 
%%				
				
% Use Agrawal Anderson for finding first DFS tree in $O(\sqrt{n})$ time./ or use the tree after first update.
% Make the data structure on the tree using $O(m)$ processors using $\tilde{O}(1)$ time.
% Reduce the problem to just solving reroot of $T(r)$ in O(1) time in parallel. This can be done using O(|T(r)|) processors



==> pdfsBackup.tex <==
% NOTATAIONS:::
% \tau_c heaviest tree of the component c
% p_c  path of the component c
% T(v_H) Smallest subtree with size > n_0/2^i


\section{Rerooting a DFS tree}
\label{sec:pdfs}
%%%%% UPDATE DS QUERY SYNTAX IN PSEUDOCODE
%%%% FIGURE FOR C1 and C2P2
%%%%% Remark for O(\log^2 n) using m processors
We now describe the algorithm to reroot a subtree  $T(r_0)$ of the DFS tree $T$, 
from its original root $r_0$ to the new root $r^*$. 
Let $n_0$ denote the number of vertices in the subgraph induced by $T(r_0)$. 
Also, let the data structure $\cal D$ be built on $T$ described in Theorem \ref{thm:DS}.
%Given the current DFS tree $T$ of the graph and data structure $\cal D$ built on it, 
%the following algorithm requires $n_0$ processors 
%to perform this rerooting in $O(\log^3 n)$ time on EREW PRAM. 
Also we maintain the following invariant: at any moment of the algorithm, 
every component $c$ of the unvisited graph can be of the following two types: 

\begin{itemize}
\item[C1:] Consists a single subtree $\tau_c$ of the DFS tree $T$. 
%		   We also have a vertex $r_c\in \tau_c$ from which the DFS tree of the component $c$ 
%		   would be rooted in the final DFS tree $T^*$.
\item[C2:] Consists of a single {\em ancestor-descendant} path $p_c$ and a set 
			${\cal T}_c$ of subtrees of the DFS tree $T$ having at least one edge to $p_c$. 
%			We also have a vertex $r_c\in {\cal T}_c\cup p_c$ 
%			from which the DFS tree of the component $c$ would be rooted in the final DFS tree $T^*$. 
			Note that for any $\tau_1,\tau_2\in{\cal T}_c$, there is no edge between $\tau_1$ and $\tau_2$ since $T$ is a DFS tree.
\end{itemize}
Moreover, for every component $c$ we also have a vertex $r_c\in c$ from which the DFS tree of the component $c$ 
would be rooted in the final DFS tree $T^*$.


\newcommand{\Th}{{\mathbb{T}}}

The algorithm is divided into $\log n_0$ {\em phases}, where each phase is further divided 
into $\log n_0$ {\em stages}.
%For notational convenience, we refer to the phases as $P_0,P_1.P_2,...$ and the stages during a phase
%as $S_0,S_1,S_2,...$ . Furthermore, at the beginning of every phase and every stage, the structure of 
%every component $c$ of the unvisited graph can be of the following types:
At the end of phase $P_i$, every subtree of any component $c$ ($\tau_c$ or subtrees in ${\cal T}_c$) 
has at most $n_0/2^i$ vertices.
During phase $P_i$, every component has at least one {\em heavy} subtree (having $\geq n_0/2^{i}$ vertices). 
If no such tree exists we move the component to the next phase. We denote the set of these heavy subtrees by $\Th_c$.
% During phase $P_i$, every component has exactly one {\em heavy} subtree 
% (having $\geq n_0/2^{i}$ vertices). If no such tree exists we move the component to the next phase.
For notational convenience, we refer to the heaviest subtree of every component $c$ as 
$\tau_c$, even for components of type $C2$.
Hence, for any component of type $C1$ or $C2$, we have $\tau_c\in \Th_c$. 
Clearly the algorithm ends after $\log n_0$ phases as every component of the unvisited graph would be empty.  

At the end of stage $S_j$ of a phase, the length of $p_c$ in each component $c$ is at most $n_0/2^j$. 
If $|p_c|\leq n_0/2^{j}$, we move the component $c$ to the next stage.
Further, for any component $c$ of type $C1$, the value of $|p_c|$ is zero, 
so we move such components to the last stage of the phase, i.e., $S_{\log n_0}$. 
Clearly at the end of $\log n_0$ stages, each component would be of type $C1$.

In the beginning of the algorithm, we have the component induced by $T(r_0)$ of type $C1$ where $r_c=r^*$.
%the algorithm begins at the end of final stage $S_{\log n_0}$ of the first phase $P_1$, 
%where the component induced by $T(r_0)$ is of type $C1$ and $r_c=r^*$. 
Note that during each stage, different connected components of the unvisited graph can be 
processed independent of each other.
\textbf{Note that during each stage, different connected components of the unvisited graph can be 
processed independent of each other in parallel. 
The number of processors assigned to each component is equal to the number of vertices in the component. 
}% Thus, if each stage of the algorithm can be completed in $t$
% time, the total time taken by the algorithm is $O(t \log^2 n_0)$.
 
\subsection{Algorithm}
We shall now describe how a component $c$ in phase $P_i$ and stage $S_j$ is traversed by our algorithm.
The aim is to build a partial DFS tree for the component $c$ rooted at $r_c$, 
that can be attached to the partially built DFS tree $T^*$ of the updated graph.
Note that this has to be performed in such a manner that every component of the unvisited part of $c$
is of type $C1$ or $C2$ only.

Now, in order to move to the next phase, we need to ensure that for every component $c'$ of the unvisited part of $c$, 
$|\tau_{c'}|\leq n_0/2^i$.  After $\log n_0$ stages, every component $c'$ is reduced to a component of type $C1$.
For a component of type $C1$, we perform a {\em disintegrating traversal} of $\tau_c$ which ensures
that every component of the unvisited part of $c$ can be moved to the next phase.

During $S_j$, in order to move to the next stage, we need to ensure that for every component $c'$ of the unvisited part of $c$,
either $|p_{c'}|\leq n_0/2^j$ (moving it to next stage) or  $|\tau_{c'}|\leq n_0/2^i$ (moving it to next phase). 
The component is processed based on the location of $r_c$ in $c$ as follows.
If $r_c\in p_c$, we perform {\em path halving} which ensures the components move to the next stage.
If $r_c\in \tau\notin \Th_c$, we perform a {\em disconnecting traversal} of $\tau$ followed by {\em path halving} of $p_c$
such that the unvisited components of $\tau$ are no longer connected to residual part of $p_c$ moving them to the next phase.
The remaining components of $c$ moves to the next stage due to path halving.
%If $r_c\in T(v_H)$, we can simply perform a {\em root traversal}. 
%Finally, the most difficult case is when $r_c\in \tau_c\backslash T(v_H)$, where we perform 

Finally, the most difficult case is when $r_c\in \tau\in \Th_c$. Here, some trivial cases 
can be directly processed by the simpler cases mentioned above. For the remaining cases we perform 
{\em heavy subtree traversal} of $\tau$ such that the unvisited part of $c$ reduces to these 
simpler cases. Refer to Procedure \ref{alg:parallel_dfs} for the pseudo-code of the algorithm.
%Refer to Procedure \ref{alg:parallel_dfs} in Appendix \ref{appn:pseudocode} for the pseudo-code.


\begin{figure}[h]
	\begin{procedure}[H]
		\tcc{Let current phase be $P_i$ and current stage be $S_j$}
		$\tau_c \leftarrow$ Heaviest tree in $\TT_c$\;
		$T(v_H)\leftarrow$ Smallest subtree having size at least $n_0/2^i$\;
		\lIf{$|\tau_c|\leq n_0/2^{i}$}
		{Return Reroot-DFS($r_c,p_c,\TT_c$) in next phase}
		\lIf{$|p_c|\leq n_0/2^{j}$}
		{Return Reroot-DFS($r_c,p_c,\TT_c$) in next stage}
		\BlankLine
		\tcc{Disintegrating Traversal}
		\lIf{$p_c=\phi$ or $r_c= root(\tau_c)$}
		{Return DisInt-DFS($r_c,p_c,\TT_c$)}
		\BlankLine
		\tcc{Disconnecting Traversal}
		\lIf{$r_c\notin \tau_c$ or $r_c\in T(v_H)$}
		{Return DisCon-DFS($r_c,p_c,\TT_c$)}
		\BlankLine		
		\lIf(\tcc*[f]{Path Halving}){$r_c\in p_c$}{Return Path-Halving($r_c,p_c,\TT_c,\phi$)}
		Heavy-DFS($r_c,p_c,\TT_c$)
		\tcc*{Heavy Subtree Traversal}
		
		\caption{Reroot-DFS($r_c,p_c,\TT_c$): Traversal enters through $r_c$ 
			into the component $c$ containing a path $p_c$ and set of trees $\TT_c$.}
		\label{alg:parallel_dfs}
	\end{procedure}
\end{figure}

We now describe the different types of traversals in detail.
For any component $c$, we refer to the smallest subtree of $\tau_c$ that has more than 
$n_0/2^i$ vertices as $T(v_H)$. Since $n_0/2^{i-1}\geq |\tau_c|> n_0/2^i$, $v_H$ is unique.



%\subsection{A stage of the algorithm}
%%We shall now describe how a component $c$ of type $C2$ is processed when it enters a stage $S_j$.
%%The aim is to partially traverse $c$ such that for every component $c'$ so formed, 
%%either $|p_{c'}|\leq n_0/2^j$ (moving it to next stage) or  $|\tau_{c'}|\leq n_0/2^i$ (moving it to next phase). 
%This can be performed based on location of $r_c$ in $c$ as follows.
%If $r_c\in p_c$, this can be easily done using {\em path halving}.
%If $r_c\in \tau\notin \Th_c$, we perform a {\em disconnecting traversal} of $\tau$ from
%$r_c$ to some vertex in $p_c$ which can be handled by path halving.
%Furthermore, it ensures that the unvisited components of $\tau$ are no longer connected to 
%the unvisited part of $p_c$. 
%%If $r_c\in T(v_H)$, we can simply perform a {\em root traversal}. 
%%Finally, the most difficult case is when $r_c\in \tau_c\backslash T(v_H)$, where we perform 
%Finally, the most difficult case is when $r_c\in \tau\in \Th_c$, where we perform 
%{\em heavy subtree traversal} of $\tau$ such that the unvisited part of $c$ reduces to the 
%simpler cases mentioned above. Refer to Procedure \ref{alg:parallel_dfs} in Appendix \ref{appn:pseudocode} for the pseudo-code.
%
%\subsection{A phase of the algorithm}
%We shall now describe how a component $c$ is processed when it enters a phase $P_i$.
%The aim of each phase is to build a partial DFS tree for the component $c$ rooted at $r_c$, 
%that can be attached to the partially built DFS tree $T^*$ of the updated graph.
%However, we need to ensure that at the end of the phase, 
%$|\tau_c|\leq n_0/2^i$ for every component $c$.
%In the first $\log n_0$ stages, every component $c$ is reduced to a component of type $C1$.
%For any component $c$, let $T(v_H)$ be the smallest subtree of $\tau_c$ that has more than 
%$n_0/2^i$ vertices. Since $n_0/2^{i-1}\geq |\tau_c|> n_0/2^i$, $v_H$ is unique.
%
%
%We perform a {\em disintegrating traversal} of $\tau_c$ that makes a partial
%traversal of $T(v_H)$ ensuring that no subtree of the unvisited part of $T(v_H)$ is heavy. 
%Thus, all the components of the unvisited part of $c$ can be moved to the next phase.
%
%%Thus, at the end of the phase we need to ensure that some part of $T(v_H)$ is traversed 
%%dividing it into smaller subtrees.
%%%This is achieved by guiding the DFS traversal in such a way that the unvisited part of
%%%$c$ is divided into different components each having the heavy subtree
%%%of size at most $n_0/2^{i+1}$. 
%%This is achieved by reducing every component in the phase to a component of type $C1$ 
%%in $\log n_0$ stages. Then we perform a {\em disintegrating traversal} of the subtree as described in the 
%%following section.
%%
%%This can be achieved in $\log n_0$ stages as described in the 
%%following section.

\begin{figure}[!ht]
\centering
\includegraphics[width=\linewidth]{Figures/pdfs_eg1.pdf}
\caption{The three easier types of traversals shown in blue dotted lines,
(a) Disintegrating traversal, (b) Path Halving and (c) Disconnecting traversal.}
%\caption{The four easier types of traversals shown in blue dotted lines,
%	(a) Disintegrating traversal, (b) Path Halving, (c) Disconnecting traversal, (d) Root Traversal}
\label{fig:pdfs1}
\end{figure}


\subsubsection{Disintegrating Traversal}
\label{sec:c1}
Consider a component $c$ of type $C1$ in phase $P_i$ with the new root $r_c\in \tau_c$ 
and $n_0/2^{i-1} \geq |\tau_c| > n_0/2^i$. We first find the vertex $v_H$.
\textbf{We first find the vertex $v_H$ in parallel by comparing the size of each subtree using 
the data structure described in Theorem \ref{thm:DSx}. 
}
We perform the traversal along the tree path $path(r_c,v_H)$ adding it to $T^*$ 
(see Figure \ref{fig:pdfs1} (a)). Let $v_l$ be the LCA of $r_c$ and $v_H$ in $T$ and $r'$ be the root of $\tau_c$. 
Now, the unvisited part of $c$ consists of $path(par(v_l),r')$ (say $p$) 
and the subtrees hanging from $path(r_c,r')$ and $path(v_l,v_H)$.
Notice that $p$ is an ancestor-descendant path of $T$ and each subtree has at most $n_0/2^i$ vertices. 
Each subtree not having an edge to $p$ corresponds to a separate component of type $C1$. 
The path $p$ and the remaining subtrees (having an edge to $p$) form a component of type $C2$. 
For each component $c^*$, we also need to find the new root $r_{c^*}$ for the updated DFS tree of the component.
Using the components property, we know that this is the lowest edge from $c^*$ on the path $p^*$,
where $p^*$ is the newly attached path to $T^*$ as described above. 
Both these queries (finding an edge to $p$ and the lowest edge on $p^*$) can be answered by our data structure $\cal D$ '
(see Theorem \ref{thm:DS}) in say $t_q$ time. Thus, all these components can be identified and moved to the next phase 
(refer to Procedure \ref{alg:dfs_c1} in Appendix \ref{appn:pseudocode} for the pseudo code).

\remark{
If $r_c = r'$, this traversal can also be performed on a subtree 
from a component $c$ of type $C2$ achieving similar result. 
This is possible because no new path $p$ would be formed and we 
still get components of type $C1$ and $C2$ (being connected to a single path $p_c$).}

%%% Write Independently
%%% Input, Output(Component of type 2 in next phase), Time analysis, Space required.
%%% Model Required EREW or CRCW? If not reason or specific areas which cause this. 
%%% Keep in mind the Distributed setting as well.

%\subsection{A stage of the algorithm}
%We shall now describe how a component $c$ of type $C2$ is processed when it enters a stage $S_j$.
%The aim is to partially traverse $c$ such that for every component $c'$ so formed, 
%either $|p_{c'}|\leq n_0/2^j$ (moving it to next stage) or  $|\tau_{c'}|\leq n_0/2^i$ (moving it to next phase). 
%This can be performed based on location of $r_c$ in $c$ as follows.
%If $r_c\in p_c$, this can be easily done using {\em path halving}.
%If $r_c\in \tau\notin \Th_c$, we perform a {\em disconnecting traversal} of $\tau$ from
%$r_c$ to some vertex in $p_c$ which can be handled by path halving.
%Furthermore, it ensures that the unvisited components of $\tau$ are no longer connected to 
%the unvisited part of $p_c$. 
%%If $r_c\in T(v_H)$, we can simply perform a {\em root traversal}. 
%%Finally, the most difficult case is when $r_c\in \tau_c\backslash T(v_H)$, where we perform 
%Finally, the most difficult case is when $r_c\in \tau\in \Th_c$, where we perform 
%{\em heavy subtree traversal} of $\tau$ such that the unvisited part of $c$ reduces to the 
%simpler cases mentioned above. Refer to Procedure \ref{alg:parallel_dfs} in Appendix \ref{appn:pseudocode} for the pseudo-code.
%
%%that can be attached to the partially build DFS tree $T^*$ of the updated graph.
%%if $r_c$ belongs to $p_c$, we can move the a disintegrating traversal is perform
%%based on the type of the component. 
%%The correctness of each stage of the algorithm 
%%requires the components property to be satisfied for the newly added part of the tree $T^*$.

\subsubsection{Path Halving}
Consider a component of type $C2$ with $r_c\in p_c=path(x,y)$.
We first find the farther end of $p_c$ (say $x$, where $|path(r_c,x)|\geq |path(r_c,y)|$).
We then traverse from $r_c$ to $x$ adding $path(r_c,x)$ to the tree $T^*$ (see Figure \ref{fig:pdfs1} (b)).
The component $c'$ of type $C2$ thus formed will have $p_{c'}$ of length at most half of $p_c$. 
Now, the subtrees in $c$ having an edge to $p_{c'}$ would be a part of $c'$.
The remaining subtrees would form individual components of type $C1$. 
Again, the new root of each component can be found using $\cal D$
by querying for the lowest edge on the $path(r_c,x)$ added to $T^*$ 
(refer to Procedure  \ref{alg:dfs_c2_3} in Appendix \ref{appn:pseudocode} for the pseudo code).


\subsubsection{Disconnecting Traversal}
\label{sec:discon}
Consider a component of type $C2$ with $r_c\in \tau$ where $\tau\notin \Th_c$. 
We traverse $\tau$ from $r_c$ to reach $p_c$, which is then followed by path halving of $p_c$.
The goal is to ensure that the unvisited part of $\tau$ is not connected to the 
unvisited part of $p_c$ (say $p'$) after path halving, moving it to the next phase.
The remaining components will move to the next stage as a result of path halving.

%We now describe the disconnecting traversal of $\tau\notin \Th_c$ from $r_c$ to reach $p_c$, 
%which is then followed by path halving moving each component to the next stage or the next phase.
%Further, we ensure that the unvisited part of $\tau$ is not connected to the 
%unvisited part of $p_c$ (say $p'$) after path halving.
Now, if at least one edge from $\tau$ is present on the upper half of $p_c$,
we find the lowest edge from $\tau$ to $p_c$.
Otherwise, we find the highest edge from $\tau$ to $p_c$ (see Figure \ref{fig:pdfs1} (c)).
Let it be $(x,y)$, where $y\in p_c$ and $x\in \tau$.
This ensures that on entering $p_c$ through $y$, path halving would ensure that all the edges from $\tau$ to $p_c$
are incident on the traversed part of $p_c$ (say $p$). 

We perform the traversal from $r_c$ to $x$ similar to the {\em disintegrating traversal} along the 
tree path $path(r_c,x)$ attaching it to $T^*$. 
Since, none of the components of unvisited part of $\tau$ are connected to $p'$, 
all the components formed would be of type $C1$ or $C2$ as described in Section \ref{sec:c1}. 
However, while finding the new root of each resulting component $c'$, 
we also need to consider the lowest edge from the component on $p$.
Further, since $\tau\notin \Th_c$, size of each subtree in the resulting components is at most $n_0/2^i$.
Thus, the resultant components of $\tau$ can be moved to the next phase
(see Procedure \ref{alg:dfs_c2_2} in Appendix \ref{appn:pseudocode} for the pseudo code).

\remark{ If $r_c\in T(v_H)$, this traversal can also be performed on a $\tau\in \Th_c$ getting a similar result.
This is because each subtree in resultant components of $\tau$ will have size at most $n_0/2^i$
moving it to the next phase. 
However, if $r_c\notin T(v_H)$ the resultant component $c'$ of type $C2$ formed can
have a heavy subtree and a path $p_{c'}$ of arbitrary length.
This is not permitted as it will move the component to some earlier stage in the same phase.
}
%\subsubsection{Root Traversal}
%When $r_c\in T(v_H)$, we simply traverse to the root $r'$ of $\tau_c$ (see Figure \ref{fig:pdfs1} (d)), 
%adding $path(r_c,r')$ to $T^*$. Since, $v_H$ is covered by the traversal, all the subtrees hanging from 
%$path(r_c,r')$ have size at most $n_0/2^i$ (recall the definition of $v_H$).
%Among these, the subtrees not having the an edge to $p_c$ would thus become a 
%component of type $C1$ in the next phase.
%The remaining subtrees and the subtrees in $\TT_c\setminus \tau_c$ 
%along with $p_c$ would form a component of type $C2$ in the next phase. 
%Again, the new root of each component can be found using $\cal D$
%by querying for the lowest edges on the $path(r_c,r')$ added to $T^*$ 
%(refer to Procedure  \ref{alg:dfs_c2_3} in Appendix \ref{appn:pseudocode} for the pseudo code).



\subsubsection{Heavy Subtree Traversal}
Consider a component $c$ of type $C2$, where $r_c\in\tau$ where  $\tau \in \TT_c$ and $r'$ is the root of $\tau$.
As described earlier, if $r_c$ is the root of $\tau$ or $r_c\in T(v_H)$ it can be processed using 
disintegrating or disconnecting traversals respectively. 
Otherwise, the heavy subtree $\tau$ can be traversed using a combination of disintegrating and disconnecting traversals
such that every unvisited component of $c$ can be moved to the next phase.
We first perform a disintegrating traversal of $\tau$, which leads to formation of another path, i.e., 
the unvisited part of $path(r_c,r')$ in addition to the path $p_c$ in the component.
Hence, the newly formed component is neither of type $C1$ nor $C2$. 
Thus, the aim of the remainder of this traversal is to make sure $p_c$ is completely traversed
so that the components of the unvisited part of $c$ are of types $C1$ and $C2$ in the next phase.

We shall refer to $p_c$ as the \textit{primary} path and the unvisited part of
$path(r_c,r')$ as the \textit{secondary} path of the component. Moreover, we shall see 
shortly different subtrees in the component $c$ may have different secondary paths but a unique
primary path $p_c$. As a result the component will eventually have many secondary paths in $P_c$
and one primary path $p_c$ such that each subtree on $\TT_c$ is connected to at most one secondary path. 
Let $\TT_{c_i}$ represent the set of subtrees in $\TT_c$ connected to secondary path $p_i\in P_c$.

Now, as described earlier heavy path traversal of $\tau\in \TT_c$ creates a secondary path $p_i$
and all the unvisited subtrees of $\tau$ are added to $\TT_{c_i}$. As we know whenever the 
traversal enters $p_c$ it is reduced to half as a result of path halving. Now, whenever $r_c\in \TT_{c_i}$
the traversal can reach $p_c$ using $O(\log n)$ disconnecting traversals described as follows. 
Let $r_c\in \tau \in \TT_{c_i}$, we perform a disconnecting traversal of $\tau$ disconnecting it from the
secondary path $p_i$. As a result the unvisited parts of $\tau$ will not be connected to $p_i$ but can still be
connected to $p_c$ and a new path $p_j$ produced as a result of the disconnecting traversal. Thus, these 
subtrees would be transferred to $\TT_{c_j}$. Now, we can have three cases based on the location of 
the new root of the unvisited part of $c$, i.e., $r'_c$. \textit{Firstly}, if $r'_c\in p_c$, 
the traversal has simply reached $p_c$ in a single step. \textit{Secondly}, if $r'_c\in p_i\cup \TT_{c_i}$,
we simply repeat the disconnecting traversal to $p_i$. This step can clearly occur only $O(\log n)$ times 
as $p_i$ is reduced to half during every disconnecting traversal. \textit{Finally}, if $r'_c\in \TT_{c_j}$,
this can happen only if $p_j\cup \TT_{c_j}$ has the lowest edge on the traversed part of $p_i$ among $\TT_{c_j},\TT_{c_i}$ and $p_c$.
Let this edge be $(x,y)$ where $x\in \tau$ and $y\in p_i$. In such a case we do not perform the previous disconnecting
traversal of $\tau$, rather we traverse $\tau$ along $path(r_c,x)$ to reach $p_i$ at $y$ and traverse $p_i$ using path halving.
The unvisited part of $p_i$ will now be disconnected from all subtrees as well as $p_c$. We can thus treat it as a component $C_2$
in the next phase. All the remaining subtrees in $\TT_{c_i}$ will now be connected only to $p_c$ and thus have no secondary path.
It will thus reach $p_c$ using a single disconnecting traversal.
Note that there still may be other subtrees in $\TT_{c_k}$'s connected to $p_c$ having a secondary paths. All these subtrees will
perform in similar way until the phase ends and $p_c$ becomes empty. As a result each $\TT_{c_k}$ would be converted to a component of type $C2$.   



\subsubsection{Heavy Subtree Traversal}
Consider a component $c$ of type $C2$, where $r_c\in\tau$ where  $\tau \in \TT_c$.
As described earlier, if $r_c$ is the root of $\tau$ or $r_c\in T(v_H)$ it can be processed using 
disintegrating or disconnecting traversals respectively. 
Otherwise, the heavy subtree $\tau$ can be traversed using one of three scenarios described as follows (see Figure \ref{fig:pdfs}).
Our algorithm checks each scenario in turn for its applicability to $\tau$, 
eventually choosing a scenario and perform a $l,p$ or $r$ traversal (described below) 
which is followed by a {\em disconnecting traversal}.
Thus, each component will move to the next phase or the next stage as described in Section \ref{sec:discon}.
We shall also prove that these scenarios are indeed exhaustive, i.e., for any $\tau$, one of the scenarios 
is indeed applicable moving the component to the next stage/phase.


\textbf{Each of the traversals described earlier requires $O(1)$ steps 
to move to the next stage/phase. In order to achieve the same for heavy subtrees 
in $\TT_c$, we describe three scenarios for traversing a heavy subtree $\tau$ (see Figure \ref{fig:pdfs}).
Our algorithm checks each scenario in turn for its applicability to $\tau$ in
$O(1)$ steps, eventually choosing a scenario that will lead to a {\em disconnecting traversal} in $O(1)$ steps.
 We shall prove that these scenarios are indeed exhaustive, i.e., for any $\tau$, the traversal 
can be done using one of these scenarios in $O(1)$ steps to reach the next stage/phase.
}

We now present a few notations related to $\tau\in \Th_c$ that shall be used in the rest of the section. 
Let $r'$ be the root of $\tau$, and $T(v_h)$ be the subtree hanging from $path(r_c,r')$ containing $v_H$
(see Figure \ref{fig:pdfs}). Note that $v_h$ can always be defined as $r_c\notin T(v_H)$. 
%otherwise we simply perform a {\em disconnecting traversal} of $\tau$ to move to the next stage 
%(see Remark in Section \ref{sec:discon}).

\begin{figure}[!ht]
	\centering
	\includegraphics[width=\linewidth]{Figures/pdfs_eg.pdf}
	\caption{The three scenarios for Heavy Subtree Traversal (blue dotted lines) showing (a) $l$ traversal, 
	(b) $p$ traversal and (c) $r$ traversal.
%		(a) The $\mathbb{L}$ traversal, (b) The $\mathbb{P}$ traversal and (c) The $\mathbb{R}$ traversal.
		}
	\label{fig:pdfs}
\end{figure}


\begin{scenario}
\end{scenario}
Consider the $l$ traversal shown in Figure \ref{fig:pdfs} (a).
%This traversal shall be followed by a disconnecting traversal of some subtree $\tau'$
%hanging from $path(r_c,r')$. This is possible if $\tau'$ has an edge to $p_c$ and the 
%highest edge (say $(x',y')$ where $x'\in \tau$) among such subtrees to $path(r_c,r')$ (components property).
%However, this scenario is applicable only if $\tau'\neq T(v_h)$ or $x'\in T(v_H)$ (see disconnecting traversal).
%Otherwise, we shall move to check the next scenario. We now describe how this check is performed
%also querying some information to be used in the later scenarios.
%
We first find the highest edge on $path(r_c,r')$ from subtrees hanging from it
and having an edge to $p_c$. Let this edge be $(x',y')$, where $y'\in path(r_c,r')$ and 
the corresponding subtree be $\tau'$. This scenario is applicable only if we can perform a disconnecting traversal
through the subtree $\tau'$ using the root $x'$, i.e., $\tau'\neq T(v_h)$ or $x'\in T(v_H)$ 
(see Remark in Section \ref{sec:discon}).
In such a case,  all the other subtrees (except $\tau'$) hanging from $path(r_c,r')$ and connected to $p_c$ 
move to the next stage as a component of type $C2$. The remaining subtrees represent a component of type $C1$.
However, if this scenario is not applicable we perform the query again in a different manner
described as follows. The results of this query shall be used in the future scenarios. 

We find the highest edge on $path(r_c,r')$ from subtrees hanging from it
(except $T(v_h)$) and subtrees hanging from $path(v_h,v_H)$,
considering only those subtrees that have an edge to $p_c$.
Let this edge be $(x,y)$, where $y\in path(r_c,r')$. 
We store this edge as $(x^*,y^*)$ to be used in the Scenario 3.

We now have two cases. Case A: $x\in T(v_h)$ or Case B: $x\notin T(v_h)$.
Case B is possible if $x'$ (in the previous query) belongs to
some subtree hanging from $path(v_h,v_H)$ that does not have
an edge to $p_c$ or $x'\in path(v_h,v_H)$. 
For Case B, we perform the same query again without the restriction of having an edge to $p_c$.
Let the edge be $(x,y)$. If still $x\notin T(v_h)$ it means that $x'\in path(v_h,v_H)$.
We then use $(x',y')$ as $(x,y)$. 

Now, if $(x,y)$ is a tree edge (i.e. $(v_h,par(v_h))$), 
we simply perform {\em disintegrating traversal} of $T(v_h)$ (see Remark in Section \ref{sec:c1}).
As a result, the unvisited subtrees of $\tau$ will no longer be heavy.
Also, $r_c'$ for the components so formed would be in the unvisited subtrees of $\tau$.  
This leads to one of the easier traversals described earlier.
Otherwise, we have a back edge $(x,y)$ of $T$ from $T(v_h)$ to $path(r_c,r')$
which shall be used in Scenario 2.

\begin{scenario}
\end{scenario}
Consider the $p$ traversal shown in Figure \ref{fig:pdfs} (b).
Let $T(v_{h_1})$ be the subtree hanging from $path(v_h,x)$ that contains $T(v_H)$.
Let $p$ be the traversed path, i.e., $p\leftarrow path(r_c,x)\cup (x,y) \cup path(y,par(par(v_h)))$.
Find the lowest edge from the subtrees hanging from $path(r_c,r')$ (except $T(v_h)$)
and $path(v_h,x)$ to $p$. Let this edge be $(x_1,y_1)$.

Again, if $x_1\in T(v_H)$ or $x_1\notin T(v_{h_1})$, we perform a 
{\em disconnecting traversal} of the corresponding subtree through the root $x_1$.
We add $p$ and the edge $(y_1,x_1)$ to $T^*$ that will 
be followed by the above mentioned disconnecting traversal.
Note that this may leave an unvisited path $path(par(y),r')$, which is not 
connected to any subtree queried in previous scenario. Hence, it is not connected to $p_c$
and the corresponding component can be moved to the next phase with $r_c$ given 
by lowest edge from the component on the traversed path.

%Otherwise, $x\in T(v_{h_1})\backslash T(v_H)$. 
Now, if $(x_1,y_1)$ is a tree edge (i.e. $(v_{h_1},par(v_{h_1}))$), 
we simply perform {\em disintegrating traversal} of $T(v_{h_1})$ (similar to Scenario 1)
leading to one of the easier traversals.
%
%However, if $(x_1,y_1)=(v_{h_1},par(v_{h_1}))$,
%we simply perform a disintegrating traversal of $T(v_{h_1})$ (see Remark in Section \ref{sec:c1})
%followed by one of easier traversals described before 
%as $T(v_H)$ has disintegrated.
Otherwise, we move to the next scenario, where we have two back edges $(x,y)$ and $(x_1,y_1)$ 
from $T(v_h)$ to $path(r_c,r')$ such that $x_1\in T(v_{h_1})$ and $x\in T(v_h)$.

\begin{scenario}
\end{scenario}
Consider the $r$ traversal shown in Figure \ref{fig:pdfs} (c).
We shall show that this scenario is always applicable if Scenario 1 and Scenario 2 are not.
%We shall now show that this scenario shown in Figure \ref{fig:pdfs} (c) is always applicable.
We traverse $path(r_c,x_1)$ and using $(x_1,y_1)$ enter $path(y_1,r')$ to traverse it completely.
Now, we prove that the disconnecting traversal can always be performed using the edge $(x^*,y^*)$.
Recall the components property, we need to prove that $(x^*,y^*)$ is the lowest edge on the traversed path.
Recall the query for finding $(x^*,y^*)$, let the subtree containing $x^*$ in the first query be $\tau$.
If $x^*\in T(v_h)$ (case A), then $x^*$ does not lie on $path(v_h,v_H)$.
Since $x_1\in T(v_{h_1})$, $path(v_h,x_1)$ would follow $path(v_h,v_H)$ at least till 
$par(root(\tau))$. Thus, $\tau$ would still be the highest subtree with an edge to $p_c$ on the 
path as shown in Figure\ref{fig:pdfs} (c).
If $x^*\notin T(v_h)$ (case B), then no subtree on $path(v_h,x_1)$ having edge to $p_c$ can have and edge higher 
than $\tau$ on $path(r_c,r')$, otherwise $(x^*,y^*)$ would not have the highest edge back then.
Thus, in both cases A and B, this scenario is applicable followed by disconnecting traversal using $(x^*,y^*)$
(refer to Procedure \ref{alg:dfs_c2} in Appendix \ref{appn:pseudocode} for the pseudo code).
The reader is advised to verify that, without the seemingly unintuitive computation of $(x,y)$ in Scenario 1,  $(x^*,y^*)$ would not always be the highest edge leading to disconnecting traversal as claimed above.



%We first find the highest edge $(x,y)$ on $path(r_c,r')$ from subtrees hanging from it
%(except $T(v_h)$) and subtrees hanging from $path(v_h,v_H)$. 
%We consider only those subtrees that have an edge to $p_c$.
%Let this edge be $(x,y)$, where $y\in path(r_c,r')$. We store this edge as $(x^*,y^*)$ to be used in the last step.
%Now, we have two cases before we move to the next step.
%
%In case $x\notin T(v_h)$, (lowest for Fig \ref{fig:pdfs} (a) can still be in $T(v_h)$ as whole of it not queried)
%we perform another check before making a {\em disconnecting} traversal through it to halve $p_c$, 
%ending the stage (see Figure \ref{fig:pdfs}(a)).
%
%Firstly, if $T(v_h)$ does not have an edge to $p_c$ ($T(v_h)$ no longer eligible for lowest edge in case (a)),
%we simply add $path(r_c,r')$ and edge $(x,y)$ to $T^*$ moving to part two, with new root $x$. This ensures that new $\tau_c$ would move to the final stage of the phase.
%
%
%Else, We find the highest edge on $path(r_c,r')$ from subtrees hanging from $path(v_h,v_H)$ without 
%having an edge to $p_c$ (since ones with edges in $p_c$ not high enough). 
%If no such edge is higher than $y$, we find such an edge from entire $T(v_h)$
%(this might be possible if edge is on $path(v_h,v_H)$). 
%In case we find such an edge, we call it $(x,y)$ and move to next step.
%(both of these cases UNSOLVED. Highest in (a) belong to $T(v_h)$ but cannot be exploited 
%for (c) ).
%
%
%Now, if $x\in T(v_H)$ or we did not find the edge as described above (lowest edge not
%in $T(v_h)$ connected to $p_c$), we perform a {\em disconnecting} traversal through the edge 
%(as shown in Figure \ref{fig:pdfs}(a)) by adding $path(r_c,y)$ to the tree $T^*$ and 
%leaving through $(y,x)$ in part 2.
%(Disconnecting traversal better than root traversal in case multiple $\tau_c$ exist).
%
%Note that this may leave an unvisited path $path(par(y,r')$, which however is not 
%connected to any subtree first queried during this step. Hence, it is not connected to $p_c$
%and the corresponding component can be moved to the next phase with $r_c=par(y)$.
%
%Hence, for the next step we have an edge $(x,y)$ from $T(v_h)$ to $path(r_c,r')$.\\
%(the lowest edge is (x,y) in $T(v_h)$, best case exploiting (c) if $(x*,y*)$ available).
%


%%\subsubsection{Component type 2}
%
%
%%Consider a component $c$ of type $C2$ in phase $P_i$ and stage $S_j$. 
%%Thus, $c$ is the subgraph induced by an ancestor-descendant path $p_c$ and 
%%some subtrees of $T$ with the heaviest subtree $\tau_c$ such that 
%%$n_0/2^{j+1} \leq |p_c| < n_0/2^j$ and $n_0/2^{i+1} \leq |\tau_c| < n_0/2^i$.
%%We are required to perform the DFS traversal of this subgraph
%%from the vertex $r_c$ in $\tau_c$ such that each component $c'$ of the unvisited part of $c$ 
%%either has  $|\tau_{c'}|\leq |\tau_c|/2$ (moving to the next phase) or $|p_{c'}|\leq |p_c|/2$ (moving to the next stage). 
%%
%%
%%Now, we shall describe the three parts in which this stage is completed.
%%However, in order to explain the intuition behind the approach we shall describe these parts in the 
%%reverse chronological order. A component can also start directly in the second or third part
%%as described below.
%
%\begin{itemize}
%
%
%
%
%\item \textbf{Part 1:} When $r_c \in \tau_c$:
%
%Note that the {\em disconnecting} traversal cannot be performed in $\tau_c$ 
%as in the resulting component $c'$ disconnected from $p_c$ can have a heavy subtree 
%(more than $n_0/2^{i+1}$ vertices) with the new path $p_{c'}$ of arbitrary large length
%(as compared to $p_c$).
%We now present a few notations that shall be used in the rest of the section to denote some parts of 
%$\tau_c$. Let $r'$ be the root of $\tau_c$, and $T(v_h)$ be the heaviest subtree hanging from $path(r_c,r')$.
%
%This part is performed in three steps. In each step, the traversal would follow the path as described 
%in Figure \ref{fig:pdfs} in certain cases, in the other cases it would move to the next step.\\
%
%%\begin{case}
%%Highest edge on $r_c$ to $r'$ from subtrees hanging on the $path(r_c,r')$.
%%Follow the path from $r_c$ to $r'$ 
%%\end{case}
%%Prob: Lowest edge $(x,y)$ in $T(v_h)$.
%
%\begin{step}
%	\textbf{Traversal of the form Figure \ref{fig:pdfs} (a).}
%\end{step}
%We first find the highest edge on $path(r_c,r')$ from subtrees hanging from it (except $T(v_h)$)
%and subtrees hanging from $path(v_h,v_H)$. We consider only those subtrees that have an edge to $p_c$.
%Let this edge be $(x,y)$, where $y\in path(r_c,r')$. We store this edge as $(x^*,y^*)$ to be used in the last step.
%Now, we have two cases before we move to the next step.
%
%In case $x\notin T(v_h)$, we perform another check before making a {\em disconnecting} traversal 
%through it to halve $p_c$, ending the stage (see Figure \ref{fig:pdfs}(a)).
%Firstly, if $T(v_h)$ does not have an edge to $p_c$, we simply add $path(r_c,r')$ and edge $(x,y)$
%to $T^*$ moving to part two, with new root $x$. This ensures that new $\tau_c$ would move to the 
%final stage of the phase.
%Otherwise, We find the highest edge on $path(r_c,r')$ from subtrees hanging from $path(v_h,v_H)$ without 
%having an edge to $p_c$. 
%If no such edge exist we find such an edge from entire $T(v_h)$
%(this might be possible if edge is on $path(v_h,v_H)$). In case we find such an edge, we call it $(x,y)$
%and move to next step.
%
%Now, if $x\in T(v_H)$ or we did not find the edge as described above, we perform a 
%{\em disconnecting} traversal through the edge (as shown in Figure \ref{fig:pdfs}(a)).
%by adding $path(r_c,y)$ to the tree $T^*$ and leaving through $(y,x)$ in part 2.
%Note that this may leave an unvisited path $path(par(y,r')$, which however is not 
%connected to any subtree first queried during this step. Hence, it is not connected to $p_c$
%and the corresponding component can be moved to the next phase with $r_c=par(y)$.
%
%Hence, for the next step we have an edge $(x,y)$ from $T(v_h)$ to $path(r_c,r')$.\\
%
%\begin{step}
%	\textbf{Traversal of the form Figure \ref{fig:pdfs} (b).}
%\end{step}
%Let $T(v_{h_1})$ be the subtree hanging from $path(v_h,x)$ that contains $T(v_H)$.
%Find the lowest edge from the subtrees hanging from $path(r_c,r')$ (except $T(v_h)$)
%and $path(v_h,x)$ to $path(y,par(v_h))$. Let this edge be $(x_1,y_1)$.
%
%Now, if $x\in T(v_H)$ or $x\notin T(v_{h_1})$, we perform a 
%{\em disconnecting} traversal through the edge (as shown in Figure \ref{fig:pdfs}(b))
%by adding $path(r_c,x)\cup path(y,par(v_h))$ to the tree $T^*$ and leaving through $(y_1,x_1)$
%in part 2.
%Note that this may leave an unvisited path $path(par(y),r')$, which however is not 
%connected to any subtree first queried during this step. Hence, it is not connected to $p_c$
%and the corresponding component can be moved to the next phase with $r_c$ given 
%by lowest edge from the component on $path(y,r_c)$.
%
%Otherwise, we move to the next step, where we have two edges $(x,y)$ and $(x_1,y_1)$
%from $T(v_h)$ to $path(r_c,r')$ such that $x_1\in T(v_{h_1})$.\\
%
%\begin{step}
%	\textbf{Traversal of the form Figure \ref{fig:pdfs} (c).}
%\end{step}
%We shall now use the edge $(x^*,y^*)$ stored in the first step to perform traversal as follows.
%We follow the path $path(r_c,x_1)$ then using $(x_1,y_1)$ to enter $path(y_1,r')$ and later exit through $(x^*,y^*)$.
%Now, in order to prove that this path indeed satisfies the components property consider the following arguments.
%Recall the query for finding $(x^*,y^*)$, let the subtree containing $x^*$ in the first query be $\tau$.
%If $x^*\in T(v_h)$ then it does not lie on $path(v_h,v_H)$.
%Now, as $x_1$ belonged to $T(v_{h_1})$, $path(v_h,x_1)$ would follow $path(v_h,v_H)$ at least till $root(\tau)$.
%Thus, $\tau$ would still be the highest subtree with an edge to $p_c$ on the path as shown in Figure\ref{fig:pdfs} (c).
%If $x^*\notin T(v_h)$, then no subtree on $path(v_h,x_1)$ having edge to $p_c$ can have and edge higher 
%than $\tau$ on $path(r_c,r')$, otherwise $\tau$ would not have the highest edge back then.
%Refer to Procedure \ref{alg:dfs_c2} in Appendix \ref{appn:pseudocode} for the pseudo code of this part of the algorithm.
%
%
%\end{itemize}

\subsubsection*{Correctness:}
To prove the correctness of our algorithm, it is sufficient to prove two properties.
\textit{Firstly}, the components property is satisfied in each traversal mentioned above.
\textit{Secondly},  every component in a phase/stage, 
abides by the size constraints defining the phase/stage.
%To prove the correctness of the algorithm we need to ensure that the components
%property is satisfied in each traversal mentioned above.
%A We also need to ensure that every component in a phase/stage, 
%abides by the size constraints defining the phase/stage.
By construction we always choose the lowest edge from a component to the 
recently added path in $T^*$ ensuring that the components property is satisfied.
Furthermore, in the different traversals we have clearly proved how the 
stage/phase is progressed ensuring the size constraints.
Thus, the final tree $T^*$ returned by the algorithm is indeed the 
DFS tree of the updated graph.

\subsubsection*{Analysis:}
We now analyze the time required by each stage of the algorithm for processing a component $c$.
Every traversal described above uses $O(1)$ steps to move every component to the next phase/stage 
(refer to Appendix \ref{appn:pseudocode} for the pseudo code).
Further, every instruction of the algorithm (excluding queries on $\cal D$) 
can be performed in $O(\log n)$ time using $|c|$ processors (see Section \ref{sec:prelim}).
%Every instruction of the algorithm (refer to Appendix \ref{appn:pseudocode} for the pseudo code)
%including the data structure queries, can be performed in $O(\log n)$ time using 
%$|c|$ processors (see Section \ref{sec:prelim}).
The queries on $\cal D$ of the type $Query(T(w),path(x,y))$ require $|T(w)|$ processors 
and queries of the type $Query(path(u,v),path(x,y))$ require 
$\max(|path(v,w)|,|path(x,y)|)$ processors (using Theorem \ref{thm:DS}). 
However, since each set of parallel data structure queries include at most one path query 
($p_c$ for a component $c$), the overall $c$ processors would suffice to perform these queries
Finally, for different components all the data structure queries are 
performed on different memory cells abiding the constraints of an EREW PRAM. 
%Also, the minimum/maximum of a set of numbers and hence the lowest/highest edge 
%from a set of edges can be computed in $O(\log n)$ time
%using $n$ processors (refer to Theorem \ref{thm:sort} in Appendix \ref{sec:ds}). 
Hence, overall each stage perform $O(1)$ parallel instructions requiring $O(\log n)$ time 
using $n$ processors. In the light of Theorem \ref{thm:convert}, 
since our algorithm completes in $\log n$ phases each requiring $\log n$ stages 
we have the following theorem .

\begin{theorem}
	Given an undirected graph with the data structure $\cal D$ build on its DFS tree, 
	for any given update in the graph the updated DFS tree can be computed in $O(\log^3 n)$ 
	time using $n$ processors on an EREW PRAM model. 
	\label{thm:reroot}
\end{theorem}

Thus, we can use Theorem \ref{thm:DS} and Theorem \ref{thm:reroot} to prove Theorem \ref{main-result}
and result for Parallel Fault tolerant DFS in Section \ref{sec:results}.
Furthermore, Theorem \ref{thm:reroot} can also be used to develop a distributed algorithm (refer to Appendix \ref{sec:distributed} for details) 
proving our result for Distributed Fully Dynamic DFS in Section \ref{sec:results}.

%\subsubsection{Rest}
%% Overall statement of a phase with time, space and dependence (EREW/CRCW)
%% Overall statement of Reroot and hence dynamic DFS, time, space, proc, EREW/CRCW.
%% Keep in mind the Distributed setting as well.

\subsection{Converting to Parallel Fully Dynamic DFS}
Firstly, we need to build the DFS tree of the original graph. 
This can be build using the static DFS algorithm \cite{Tarjan72} 
or any advanced parallel algorithm \cite{GoldbergPV88,AggarwalA88}.
Now, whenever the graph is updated we first build the data structure $\cal D$ 
on the existing DFS tree in $O(\log n)$ time using $O(m)$ processors (Theorem \ref{thm:DS}). 
We then convert the graph update into appropriate rerooting procedure computing the
final DFS tree in $O(\log^3 n)$ time using $O(n)$ processors (Theorem \ref{thm:reroot}).
We can similarly process any future updates using the current DFS tree.
This proves our result for fully dynamic maintenance of DFS tree on an EREW PRAM described in Section \ref{sec:results}.
%Thus, we have the following theorem

%\begin{theorem}
%	Given any arbitrary online sequence of vertex or edge updates, 
%	we can maintain a DFS tree in $O(\log^3 n)$ time per update 
%	using $m$ processors in parallel EREW model.
%\end{theorem}




%%\noindent BUILDING LCA STRUCTURE NOT SUPPORTED IN O(1) time
%%\textbf{Note: } The cost of answering data structure queries adds a $O(\log n)$ factor to the update time.
%% In CRCW model, the LCA queries are answerable in $O(1)$ time, whereas queries on $\cal D$ can be performed 
%% in $O(1)$ time by using $m$ processors in priority CRCW model replacing the binary search (see Appendix \ref{sec:ds}). Thus, the result can be improved to $O(\log^2 n)$ time per update using $m$ processors in a CRCW PRAM. 
%%				
				
% Use Agrawal Anderson for finding first DFS tree in $O(\sqrt{n})$ time./ or use the tree after first update.
% Make the data structure on the tree using $O(m)$ processors using $\tilde{O}(1)$ time.
% Reduce the problem to just solving reroot of $T(r)$ in O(1) time in parallel. This can be done using O(|T(r)|) processors


